Three-Way Dissection of a Game-CAPTCHA: Automated Attacks, Relay Attacks, and Usability

Existing captcha solutions on the Internet are a major source of user frustration. Game captchas are an interesting and, to date, little-studied approach claiming to make captcha solving a fun activity for the users. One broad form of such captchas -- called Dynamic Cognitive Game (DCG) captchas -- challenge the user to perform a game-like cognitive task interacting with a series of dynamic images. We pursue a comprehensive analysis of a representative category of DCG captchas. We formalize, design and implement such captchas, and dissect them across: (1) fully automated attacks, (2) human-solver relay attacks, and (3) usability. Our results suggest that the studied DCG captchas exhibit high usability and, unlike other known captchas, offer some resistance to relay attacks, but they are also vulnerable to our novel dictionary-based automated attack.

==> discussion.tex <==
\section{Discussion}
\label{sec:discuss}

% Taking Everything together -- automated, relay and usability -- insights
% The main message
% How to improve security and usability of DCG CAPTCHA



% Other categories of DCG CAPTCHA -- moving target and specific path games
% Any other categories?



%% Effect of background, type of objects, etc.


%% Effect of Training on Relay Experiment



%% Porting to Mobile Devices



%% Game CAPTCHA based on hard AI problems -- Go game








==> relay-user-compressed.tex <==
%\section{Usability}
%
%\label{sec:usability}

In this section, we report on a usability study of DCG captcha, including the
study design, goals, and testing process, as well as study results.

\subsection{Study Design, Goals and Testing Process}

Our study was undertaken by 40 participants. The corpus of participants
comprised primarily of undergraduate and graduate students from various
backgrounds. The demographics of the participants are shown in Table
\ref{tab:demographics-interviews}. The study was \textit{web-based} and
comprised of three phases. The \textit{pre-study phase} involved registering
and briefly explaining the participants about the protocols of the study.  In
particular, the participants were shown ``consent information,'' which they had
to agree before proceeding with the study.  This was followed by collecting
participant demographics and then the participants playing the different DCG
captcha games.  This \textit{actual study phase} attempted to mimic a realistic
captcha scenario which typically involves filling out a form followed by
solving captcha. To avoid explicit priming, however, we did not mention that
the study is about captcha or security, but rather indicated that it is about
assessing the usability of a web interface.  The final, \textit{post-study
phase} required the participants to respond to a few questions about their
experience and feedback on the games they played as part of the interface. This
included some questions on the usability of games and SUS. 

%The scenario given for study required users to evaluate a new interface for
%registering for a website followed by playing 20 games. 
During the acutual study phase, each participant was asked to play 20
variations of the four DCG captcha categories implemented as discussed in Section
\ref{sec:design}. 
These variations were aimed at understanding how different parameters, i.e., object speed and
number of objects per game, affect the DCG captcha solving capability of the users. 
The order of the games presented to the participants were
counter-balanced for learning effects using the Latin Square design (a 20 x 20
Latin Square was used).
%These were presented to each participant using Latin square methodology. 
%We were not required to go through an IRB approval process before conducting
%the experiments. However, authors of this paper have previously been involved
%in studies with U.S. Institutional Review Board (IRB) approvals, and have
%applied similar practices in this study.  

%\begin{table}[htdp]
%{\footnotesize{
%\caption{Demographics of the participants.}
%\begin{center}
%\small
%\begin{tabular}{|p{5cm}| r |}
%%\rowcolors {1}{orange!35 }{ }
%\hline
%\textbf{}& \textbf{N=40} \\
%\hline
%\hline
%%\textbf{Participants}& 16 & 20 \\
%%\hline
%%\hline
%\textbf{Gender} & \\
%\hline
% Male &7 \\
% \hline
%Female&9 \\
%\hline
% \hline
%\textbf{Age} & \\
%\hline
%
%less than 18 &0 \\
%\hline
%18 - 24 &3 \\
% \hline
% 25 - 35 &1 \\
%  \hline
%35 - 50  &4\\
%  \hline
%50 - 65  &4\\
% \hline
%  \hline
%\textbf{Education} & \\
%\hline 
%Highschool &3 \\
% \hline
%Bachelors  &8  \\
% \hline
%Masters &5 \\
%\hline
%Ph. D. & 8 \\
% \hline
%  \hline
%\textbf{Profession / field of study} & \\
%  \hline
%Computer Science & 3\\
%  \hline
%Engineering &6 \\
% \hline
%Medicine & 7 \\
% \hline
% Science, Pharmaceuticals & 4\\
% \hline
%%Have a Webmail account & & \\
% Law &\\
% \hline
%Social sciences  & 8\\
%  \hline
% Others  & 8\\
%  \hline
%\end{tabular}
%\normalsize
%\end{center}
%\label{tab:demographics-interviews}
%}}
%\end{table}

The specific goal of our usability study was to evaluate and compare different DCG captcha games with
respect to the following factors:

\begin {enumerate}


\item {\textit{Efficiency}: time taken to complete each game}
\item {\textit{Robustness}: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts.}
\item {\textit{User Experience}: quantitative SUS ratings and qualitative feedback from the participants.}
\item \textit{Effect of Game Parameters}: the effect of the number of object and objects speeds on completion time and error rates

\end {enumerate}

%Our study was conducted in a variety of campus venues including: student
%laboratories, cafes, student dorms/apartments, classrooms, of�ce spaces and
%outdoor terraces .  After giving a brief overview of our study goals, we asked
%the participants to �ll out the background questionnaire to collect demographic
%information. This followed by a series 20 games to be played by the
%participants.Each user was asked to follow on-screen instructions in completing
%each task and was given a compensation of INR 75 for participating in the
%study.  
For each tested game, completion times, errors, actions and the playcount,
i.e., number of attempts made to successfully complete the games were
established, and automatically logged by the our web-interface software.

\subsection{Study Results}

We now provide the results from our usability study. We
first consider various mechanical data, i.e., time to completion and error
rates. Then, we analyze perceived qualitative aspects of the methods based on
collected user ratings. 
%We nalize our interpretations by looking at all
%measures combined.


%\begin {itemize}

\smallskip \noindent {\bf Completion Time}: Table \ref{tab:captchaeff} shows
the time taken to complete the games per game category. Clearly, all games
turned out to be quite fast, lasting for less than 10 seconds on an average
(this far lower than our time out of 1 second).  We also found that users took
maximum time to solve the Animals game with an average time of 9.25 seconds,
whereas the other games took almost half of this time.  This might have been
due to increased semantic load on the users to identify three target objects
and then match them with the corresponding answer objects. Moreover, we noticed
a significant decrease in the solving time (4.09 sec) when the target objects
were decreased to 2 (i.e., in the Shapes game), and the time was comparable to
games which had 1 target object in the challenge (the Ships game and the
Parking game). 

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Completion time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Game} &  \bf Completion Time (sec) \\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &4.94  \\
 \hline
  \raggedright{Feed the Animals} &9.25  \\
\hline
  \raggedright{Park the Boat} &4.53  \\
  \hline
  \raggedright{Match the Shapes} &5.16\\
\hline 
    \end{tabular}% For example,  
  \label{tab:captchaeff}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%


\smallskip \noindent {\bf Error Rates}:  An important result from our study is
that all the tested games yielded 100\% accuracy (overall error rate of 0\%).
In other words, none of the participant failed to complete any of the games
within the time out. This proves that DCG captchas can be highly robust in
practice.  

Next, we calculated the likelihood of exhibiting incorrect drag and drop
attempts. For example,  in the Animals game, an incorrect attempt would be to
feed the monkey with a flower instead of a banana.  We define the error rate in
this context as the number of incorrect objects (from the pool of probable
answer objects) dragged to the target area divided by the total of objects
dragged and dropped. The results are depicted in Table \ref{tab:captchaerror}.
Looking at the table, we observe that the Shape game yields the smallest error
rate with 6\% of incorrect attempts on an average for various speeds and number
of objects. This suggests that the visual matching task (as in the Shapes game)
is less error prone compared to the semantic matching task (as in the other
games).  The Shapes game error rate was marginally (by 1\%) lower than the
Ships game and the Animals game. The game challenge which seemed most difficult
for the participants to solve was the Parking game (10\% error rate). Since
this was an empty target game, with the target region and the object region
having the same background, the participants may have found it a little
difficult to perform the matching task.

\begin{table}[ht]
{\footnotesize{
 \begin{center} 
  \caption{Error  rate (incorrect attempts / total attempts) for each captcha game category.}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Game} &  \bf Error Rate (\%)\\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &6  \\
 \hline
  \raggedright{Feed the Animals} &6  \\
\hline
  \raggedright{Park the Boat} &10  \\
  \hline
  \raggedright{Match the Shapes} &5\\
\hline 
    \end{tabular}
  \label{tab:captchaerror}
 \end{center} 
}}
\vspace{-4mm}
\end{table}
%The goal of our usability study was to evaluate and compare different DCG captcha games with
%respect to the following factors:

%\begin {enumerate}
%\item {Efficiency: time taken to complete each game}
%\item {Robustness: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts }
%\item {User Experience: quantitative SUS ratings and qualitative feedback from the participants.
%\end {enumerate}item 

\smallskip
\noindent {\bf User Experience:}




\smallskip \noindent {\bf Effect of Object Speed}: Table \ref{tab:captchaspeed}
shows the performance of the games in terms of error rates and completion time
at different object speeds per game category.  To evaluate the affect of speed on performance of
the participants, we found the correlation between error rates and time taken
to solve various game at different speed levels. The correlation came to be
-0.5 showing that participants took almost same time irrespective of the error.
We also found that maximum number of errors were committed at 40 FPS speed
which demonstrate some level of difficulty for users to be able to solve the
games at faster speeds.



\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for various speed categories}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Object Speed} &  \bf Error Rate (\%)& \bf Completion Time (sec) \\
 \hline
 \hline
    \raggedright{10 FPS } &5 &6.14 \\
 \hline
  \raggedright{20 FPS} &6 &5.31  \\
\hline
  \raggedright{40 FPS} &8 &6.13  \\
  \hline
    \end{tabular}
  \label{tab:captchaspeed}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Effect of Number of Objects}: Another aspect of the
usability analysis included testing the effect of increase in the number of
objects (noise / incorrect answer objects) on the overall game performance.
Table \ref{tab:captchaobject} summarizes the error rates and time with
different number of objects.  We found a strong correlation (0.95) between the
number of objects and completion, whereas there was no significant effect of
number of objects on error rate with correlation value of 0.32.

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different number of objects.}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Number of Objects} &  \bf Error Rate (\%) & \bf Completion Time (sec) \\
 \hline
 \hline
    \raggedright{ 6 objects / game } &8 &6.63 \\
 \hline
  \raggedright{5 objects / game} &5 &5.61  \\
\hline
  \raggedright{4 objects / game} &7 & 5.33 \\
  \hline 
    \end{tabular}
  \label{tab:captchaobject}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Summary of Analysis:} Based on our analysis, we can
conclude that the DCG captcha categories tested in this work offer very good
usability, resulting in short completion times (less than 10 sec), very low
error rates (0\% per game completion, and less than 10\% per drag and drop
attempt), and high user ratings. We also find that increasing the object speed
and number of objects is likely to negatively affect the game performance, but
up to 6 objects and up to 40 FPS speed yield a high level of usability. 




==> relay-user-v0.tex <==
%\section{Usability}
%
%\label{sec:usability}

In this section, we report on a usability study of DCG captcha, including the
study design, goals, and testing process, as well as study results.

\subsection{Study Design, Goals and Testing Process}

In the relay attack study, users were given a task to play the games through the interface which we developed. The clicks on this interface were replicated on the online game version. The study comprised of 20 participants. The corpus of participants comprised primarily of undergraduate and graduate students from various backgrounds. The demographics of the participants are shown in Table~\ref{tab:demographics-interviews}. The study design was similar to the one used in the Usability study. It comprised of three phases. The \textit{pre-study phase} involved registering and briefly explaining the participants about the protocols of the study.  In particular, the participants were shown ``consent information,'' which they had to agree before proceeding with the study.  This was followed by collecting participant demographics and then the participants playing the different DCG captcha games.  This \textit{actual study phase} attempted to mimic a realistic captcha scenario which typically involves filling out a form followed by solving captcha. To avoid explicit priming, however, we did not mention that the study is about captcha or security.  The final, \textit{post-study phase} required the participants to respond to a few questions about their
experience and feedback on the games they played as part of the interface. This included some questions on the usability of games and SUS. 

%The scenario given for study required users to evaluate a new interface for
%registering for a website followed by playing 20 games. 
During the study, each participant was asked to play 20 variations of the four DCG captcha categories implemented as discussed in Section \ref{sec:design}. These variations were aimed at understanding how different parameters, i.e., object speed and number of objects per game, affect the DCG captcha solving capability of the users. The order of the games presented to the participants were counter-balanced for learning effects using the Latin Square design (a 20 x 20 Latin Square was used).
%These were presented to each participant using Latin square methodology. 
%We were not required to go through an IRB approval process before conducting
%the experiments. However, authors of this paper have previously been involved
%in studies with U.S. Institutional Review Board (IRB) approvals, and have
%applied similar practices in this study.  

\begin{table}[htdp]
{\footnotesize{
\caption{Demographics of the participants. (All values are in percentages)}
\begin{center}
\small
\begin{tabular}{|p{5cm}| r |}
%\rowcolors {1}{orange!35 }{ }
\hline
\textbf{}& \textbf{N=20} \\
\hline
\hline
%\textbf{Participants}& 16 & 20 \\
%\hline
%\hline
\textbf{Gender} & \%\\
\hline
 Male &70 \\
 \hline
Female&30 \\
\hline
 \hline
\textbf{Age} & \% \\
\hline
less than 18 &0 \\
\hline
18 - 24 &35 \\
 \hline
 25 - 35 &60 \\
  \hline
35 - 50  &5\\
  \hline
50 - 65  &0\\
 \hline
  \hline
\textbf{Education} & \% \\
\hline 
Highschool &25 \\
 \hline
Bachelors  &45 \\
 \hline
Masters &30 \\
\hline
Ph. D. & 0 \\
 \hline
  \hline
\textbf{Profession / field of study} & \% \\
  \hline
Computer Science & 90\\
  \hline
Engineering &5 \\
 \hline
Medicine & 5 \\
 \hline
 \end{tabular}
\normalsize
\end{center}
\label{tab:demographics-interviews}
}}
\end{table}

The relay attack study was conducted to answer and evaluate the following
\begin {enumerate}


\item {\textit{Efficiency}: time taken to complete each relay attack}
\item {\textit{Robustness}: incorrect drags to the target area}
\item {\textit{User Experience}: quantitative SUS ratings and qualitative feedback from the participants.}
\item \textit{Effect of Game Parameters}: the effect of the number of object and objects speeds on completion time and error rates
\item  {\textit{Reaction time}: Time lapse between when clicks, till the game finishes or is timed out. We also Compare these solving rates to human solving the game in a realistic scenario (as in the user study)}

\end {enumerate}

%Our study was conducted in a variety of campus venues including: student
%laboratories, cafes, student dorms/apartments, classrooms, ofÞce spaces and
%outdoor terraces .  After giving a brief overview of our study goals, we asked
%the participants to Þll out the background questionnaire to collect demographic
%information. This followed by a series 20 games to be played by the
%participants.Each user was asked to follow on-screen instructions in completing
%each task and was given a compensation of INR 75 for participating in the
%study.  
For each tested game, completion times, errors, actions and the playcount,
i.e., number of attempts made to successfully complete the games were
established, and automatically logged by the our web-interface software. In addition to this, we maintained logs of the clicks by the participants on the interface developed to 

\subsection{Study Results}

 We present various mechanical data, i.e., time to completion and error
rates for the relay attack study. We further analyze the local logs for the reaction time analysis in these relay attack technique
%We nalize our interpretations by looking at all
%measures combined.


%\begin {itemize}

\smallskip \noindent {\bf Completion Time and Error rates}: Table \ref{tab:relcaptcha} shows
the time taken to play the games per game category by different participants. Clearly, all games
turned out to be quite slower than the usability study where the games lasted for less than 10 seconds on an average
(this far lower than our time out of 1 second).  We also found that users took
maximum time to solve the Animals game with an average time of 46.50 seconds,
whereas the other games took significantly less.  This might have been
due to increased semantic load on the users to identify three target objects
and then match them with the corresponding answer objects.  We observed that the error rates were least for the ``Match the shape'' games (0.09) ; we also found it to be least in the usability study. We analyzed further the time taken by the participants for the correct games as shown in the Table \ref{tab:relcaptcha}.
\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different categories of games}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Game type} &  \bf Completion Time (sec)& \bf Error Rate  & \bf Completion time for correct games  \\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &30.92 & 0.26 &22.25 \\
 \hline
  \raggedright{Feed the Animals} &46.50 &0.40  &37.93\\
\hline
  \raggedright{Park the Boat} &28.16 &0.22  &20.45\\
  \hline
  \raggedright{Match the Shapes} &26.19 &0.09 &22.94\\
\hline 
    \end{tabular}
  \label{tab:relcaptcha}
\end{center} 
}}
\vspace{-4mm}
\end{table}%





%The goal of our usability study was to evaluate and compare different DCG captcha games with
%respect to the following factors:

%\begin {enumerate}
%\item {Efficiency: time taken to complete each game}
%\item {Robustness: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts }
%\item {User Experience: quantitative SUS ratings and qualitative feedback from the participants.
%\end {enumerate}item 


\smallskip \noindent {\bf Effect of Object Speed}: Table \ref{tab:captchaspeed}
shows the performance of the games in terms of error rates and completion time
at different object speeds per game category.  


\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for various speed categories}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Object Speed} &  \bf Error Rate (\%)& \bf Completion Time (sec) \\
 \hline
 \hline
    \raggedright{10 FPS } &0.19 &30.90 \\
 \hline
  \raggedright{20 FPS} &0.31 &30.64  \\
\hline
  \raggedright{40 FPS} &0.23 &38.62  \\
  \hline
    \end{tabular}
  \label{tab:captchaspeed}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Effect of Number of Objects}: Another aspect of the
usability analysis included testing the effect of increase in the number of
objects (noise / incorrect answer objects) on the overall game performance.
Table \ref{tab:captchaobject} summarizes the error rates and time with
different number of objects.

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different number of objects.}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Number of Objects} &  \bf Error Rate (\%) & \bf Completion Time (sec) \\
 \hline
 \hline
    \raggedright{ 6 objects / game } & &27.13 \\
 \hline
  \raggedright{5 objects / game} &0.30 &32.58  \\
\hline
  \raggedright{4 objects / game} &0.24 &30.64 \\
  \hline 
    \end{tabular}
  \label{tab:captchaobject}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf User Experience}
To understand better the feasibility of human using interfaces (as the one we developed for the relay study) for relay attack, we conducted a post survey. The survey asked the participants to share their experiences while playing the games. We also asked the SUS questions and found the score to be 49.88.  Forty five percent participants felt the games to be visually attractive and 24\% said that it was pleasurable to play the games. This number depicts high possibility of making such interfaces more usable for relay attacks and also can be thought of as an indicator of humans being able to use such interfaces for relay attack. However, most participants did not notice any change in the speed or number of objects during the attack.






















==> relay-user-v1.tex <==
%\section{Usability}
%
%\label{sec:usability}

In this section, we report on a usability study of DCG captcha, including the
study design, goals, and testing process, as well as study results.

\subsection{Study Design, Goals and Testing Process}

In the relay attack study, users were given a task to play the games through the interface which we developed. The clicks on this interface were replicated on the online game version. The study comprised of 20 participants. The corpus of participants comprised primarily of undergraduate and graduate students from various backgrounds. The demographics of the participants are shown in Table~\ref{tab:demographics-interviews}. The study design was similar to the one used in the Usability study. It comprised of three phases. The \textit{pre-study phase} involved registering and briefly explaining the participants about the protocols of the study.  In particular, the participants were shown ``consent information,'' which they had to agree before proceeding with the study.  This was followed by collecting participant demographics and then the participants playing the different DCG captcha games.  This \textit{actual study phase} attempted to mimic a realistic captcha scenario which typically involves filling out a form followed by solving captcha. To avoid explicit priming, however, we did not mention that the study is about captcha or security.  The final, \textit{post-study phase} required the participants to respond to a few questions about their
experience and feedback on the games they played as part of the interface. This included some questions on the usability of games and SUS. 

%The scenario given for study required users to evaluate a new interface for
%registering for a website followed by playing 20 games. 
During the study, each participant was asked to play 20 variations of the four DCG captcha categories implemented as discussed in Section \ref{sec:design}. These variations were aimed at understanding how different parameters, i.e., object speed and number of objects per game, affect the DCG captcha solving capability of the users. The order of the games presented to the participants were counter-balanced for learning effects using the Latin Square design (a 20 x 20 Latin Square was used).
%These were presented to each participant using Latin square methodology. 
%We were not required to go through an IRB approval process before conducting
%the experiments. However, authors of this paper have previously been involved
%in studies with U.S. Institutional Review Board (IRB) approvals, and have
%applied similar practices in this study.  

\begin{table}[htdp]
{\footnotesize{
\caption{Demographics of the participants. (All values are in percentages)}
\begin{center}
\small
\begin{tabular}{|p{5cm}| r |}
%\rowcolors {1}{orange!35 }{ }
\hline
\textbf{}& \textbf{N=20} \\
\hline
\hline
%\textbf{Participants}& 16 & 20 \\
%\hline
%\hline
\textbf{Gender} & \%\\
\hline
 Male &70 \\
 \hline
Female&30 \\
\hline
 \hline
\textbf{Age} & \% \\
\hline
less than 18 &0 \\
\hline
18 - 24 &35 \\
 \hline
 25 - 35 &60 \\
  \hline
35 - 50  &5\\
  \hline
50 - 65  &0\\
 \hline
  \hline
\textbf{Education} & \% \\
\hline 
Highschool &25 \\
 \hline
Bachelors  &45 \\
 \hline
Masters &30 \\
\hline
Ph. D. & 0 \\
 \hline
  \hline
\textbf{Profession / field of study} & \% \\
  \hline
Computer Science & 90\\
  \hline
Engineering &5 \\
 \hline
Medicine & 5 \\
 \hline
 \end{tabular}
\normalsize
\end{center}
\label{tab:demographics-interviews}
}}
\end{table}

The relay attack study was conducted to answer and evaluate the following
\begin {enumerate}


\item {\textit{Efficiency}: time taken to complete each relay attack}
\item {\textit{Robustness}: incorrect drags to the target area}
\item {\textit{User Experience}: quantitative SUS ratings and qualitative feedback from the participants.}
\item \textit{Effect of Game Parameters}: the effect of the number of object and objects speeds on completion time and error rates
\item  {\textit{Reaction time}: Time lapse between when clicks, till the game finishes or is timed out. We also Compare these solving rates to human solving the game in a realistic scenario (as in the user study)}

\end {enumerate}

%Our study was conducted in a variety of campus venues including: student
%laboratories, cafes, student dorms/apartments, classrooms, ofÞce spaces and
%outdoor terraces .  After giving a brief overview of our study goals, we asked
%the participants to Þll out the background questionnaire to collect demographic
%information. This followed by a series 20 games to be played by the
%participants.Each user was asked to follow on-screen instructions in completing
%each task and was given a compensation of INR 75 for participating in the
%study.  
For each tested game, completion times, errors, actions and the playcount,
i.e., number of attempts made to successfully complete the games were
established, and automatically logged by the our web-interface software. In addition to this, we maintained logs of the clicks by the participants on the interface developed to 

\subsection{Study Results}

 We present various mechanical data, i.e., time to completion and error
rates for the relay attack study. We further analyze the local logs for the reaction time analysis in these relay attack technique
%We nalize our interpretations by looking at all
%measures combined.


%\begin {itemize}

\smallskip \noindent {\bf Completion Time and Error rates}: Table \ref{tab:relcaptcha} shows
the time taken to play the games per game category by different participants. Clearly, all games
turned out to be quite slower than the usability study where the games lasted for less than 10 seconds on an average
(this far lower than our time out of 1 second).  We also found that users took
maximum time to solve the Animals game with an average time of 46.50 seconds,
whereas the other games took significantly less.  This might have been
due to increased semantic load on the users to identify three target objects
and then match them with the corresponding answer objects.  We observed that the error rates were least for the ``Match the shape'' games (0.09) ; we also found it to be least in the usability study. We analyzed further the time taken by the participants for the correct games as shown in the Table \ref{tab:relcaptcha}. The games showed significantly different behavior from each other (F=6.26, p=0.0007). On further analyzing the data, we found that Park the boat and Place the ship on sea  games were statistically different from each other (p=0.0005). We also found the following pair of games to be significantly different form each other - shape to ships (p=0.013), Feed the animals was significantly different form all the other three games with p$<$0.001. To compare error rates better, we investigated error rates per click i.e. for  each drag attempt whether the object being dragged was dropped at the correct position or not. The error rate / click attempt was least for the `` Place the ship'' game (0.17). This is less than `` Match the shape''  game as the number of attempted clicks by the participants for this game were less. 

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different categories of games}
        %\vspace{.2cm}
    \begin{tabular}{|p{2cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Game type} &  \bf Average Time (sec)& \bf Error Rate  & \bf Solving time &\bf Error Rate / click   \\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &30.92 (5.91) & 0.26 (0.09)&22.25 (5.04) &0.17 (0.11) \\
 \hline
  \raggedright{Feed the Animals} &46.51 (5.05)&0.40 (0.14) &37.93 (4.91) &0.65 (0.12) \\
\hline
  \raggedright{Park the Boat} &28.16 (7.36) &0.22 (0.10)  &20.45 (5.04) & 0.66 (0.12) \\
  \hline
  \raggedright{Match the Shapes} &26.19 (1.59)  &0.09 (0.07)&22.94 (1.74)&  0.56 (0.15)\\
\hline 
    \end{tabular}
  \label{tab:relcaptcha}
\end{center} 
}}
\vspace{-4mm}
\end{table}%






%The goal of our usability study was to evaluate and compare different DCG captcha games with
%respect to the following factors:

%\begin {enumerate}
%\item {Efficiency: time taken to complete each game}
%\item {Robustness: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts }
%\item {User Experience: quantitative SUS ratings and qualitative feedback from the participants.
%\end {enumerate}item 


\smallskip \noindent {\bf Effect of Object Speed}: Table \ref{tab:captchaspeed}
shows the performance of the games in terms of error rates and completion time
at different object speeds per game category.  We found not much significant difference in the variance of 3 different speeds on which the games were presented to the participants (F=2.90, p=0.06). 


\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for various speed categories}
        %\vspace{.2cm}
    \begin{tabular}{|p{2cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Object Speed} &  \bf Error Rate & \bf Error Rate / click& \bf Avg. Play Time (sec) &\bf Solving time\\
 \hline
 \hline
    \raggedright{10 FPS } &0.19 (2.06) & 0.37 (0.22)&30.90 (9.03) &24.45 (0.08) \\
 \hline
  \raggedright{20 FPS} &0.31(3.86) &0.43 (0.24)&30.64 (8.93) &30.64 (0.09) \\
\hline
  \raggedright{40 FPS} &0.23 (1.91) & 0.68 (0.23) &38.62 (10.34) &38.62 (0.10) \\
  \hline
    \end{tabular}
  \label{tab:captchaspeed}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Effect of Number of Objects}: Another aspect of the
usability analysis included testing the effect of increase in the number of
objects (noise / incorrect answer objects) on the overall game performance.
Table \ref{tab:captchaobject} summarizes the error rates and time with
different number of objects.

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different number of objects.}
        %\vspace{.2cm}
    \begin{tabular}{|p{2cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Number of Objects} &  \bf Error Rate & \bf Error Rate  / click & \bf Avg. Play Time (sec) & \bf Solving Time\\
 \hline
 \hline
    \raggedright{ 6 objects / game } &0.21 (3.3)& 0.43 (0.24) & 27.13 (10.40) &20.19 (0.05)\\
 \hline
  \raggedright{5 objects / game} &0.30 (4.08) & 0.51 (0.22) & 32.58 (8.64) &23.27 (0.08)\\
\hline
  \raggedright{4 objects / game} &0.24 (2.99) & 0.54 (0.25) & 30.64 (8.93) &24.32 (0.09) \\
  \hline 
    \end{tabular}
  \label{tab:captchaobject}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Reaction Time}
In this section, we discuss the reaction time i.e. time taken by the participants for each click on the objects. We analyzed the response time for different games during the relay attack and found that the value was least for the shape game (2.17 s) as shown in the Table~ref{tab:relay1}. The reaction time did not change drastically for any of the games. This can be used to infer that various games contributed same load on the users reflexes. Similarly, we did not notice any drastic differences on the games for variations in number of objects and speed. The reaction time was least for 10fps games (2.22 s) as shown in Table~ref{tab:relay2}. For number of objects, surprisingly the reaction time was least for games with 6 objects, this can be due more number of objects increasing users to click faster and improving detection. We found significant difference between the reaction time of the four games (F=13.19, p$<$0.01s) but for the different speeds (p=0.06) and number of objects (p=0.4), not significant difference was noticed between the games. On further analyses, we found that there was significant difference between Feed the animals (p$<$0.01) and Park the boat games (p$<$0.01).

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Reaction time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Game} &  \bf Reaction Time (sec) \\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &2.27 (0.34)\\
 \hline
  \raggedright{Feed the Animals} & 2.58 (0.35)\\
\hline
  \raggedright{Park the Boat} & 2.5 (0.51) \\
  \hline
  \raggedright{Match the Shapes} &2.17 (0.2)\\
\hline 
    \end{tabular}% For example,  
  \label{tab:relay1}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Completion time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Game} &  \bf Reaction Time (sec) \\
 \hline
 \hline
    \raggedright{10 FPS } &2.22	(0.38)\\
 \hline
  \raggedright{20 FPS } & 2.36 (0.49)\\
\hline
  \raggedright{40 FPS } &2.35 (0.07)  \\
  \hline
    \end{tabular}% For example,  
  \label{tab:relay2}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Completion time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Game} &  \bf Reaction Time (sec) \\
 \hline
 \hline
    \raggedright{ 6 objects / game } & 2.11 (0.12)\\
 \hline
  \raggedright{ 5 objects / game }&2.82 (0.33)\\
\hline
  \raggedright{ 4 objects / game } &2.36 (0.49)  \\
  \hline
    \end{tabular}% For example,  
  \label{tab:relay2}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf User Experience}
To understand better the feasibility of human using interfaces (as the one we developed for the relay study) for relay attack, we conducted a post survey. The survey asked the participants to share their experiences while playing the games. We also asked the SUS questions and found the score to be 49.88.  However, most participants did not notice any change in the speed or number of objects during the attack. 

We asked participants few likert (scale: 1 -  5) questions about their feedback on the usability of the games. Various aspects of this included - `` if the games were visually attractive'', `` Were the games pleasurable'' etc.  Forty five percent participants felt the games to be visually attractive and 24\% said that it was pleasurable to play the games. This number depicts high possibility of making such interfaces more usable for relay attacks and also can be thought of as an indicator of humans being able to use such interfaces for relay attack. The Table~\ref{tab:relaysus}, shows the average likert scores for various attributes of the game. In order to understand what stimulus worked best for the participants, we asked question about which stimulus audio, visual or both was useful as an indicator to respond fastest to the game. Thirty five percent participants found audio stimulus and visual stimulus to be sufficient where as 45\% participants agreed or strongly agreed with the statement that both visual and audio stimulus are necessary to play the game. The average score of the visual stimulus was the highest (3.20) as shown in Table~\ref{tab:relaysus}. We conducted One - way Anova, found a  variance ( F=0.64, p=0.52 ) for the three - visual, audio and both stimulus signifying no significant difference between the 3 stimuli. Eighty percent of the participants felt that training will help them play the game better with an average score of 3.95 on the likert scale. 

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Completion time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Features} &  \bf Avg. Score\\
 \hline
 \hline
    \raggedright{Visually Attractive} & 3.20 (0.92)\\
 \hline
  \raggedright{Pleasurable } & 2.85 (0.99)\\
\hline
  \raggedright{Visual Stimulus } &3.20 (1.17)\\
  \hline
   \raggedright{Audio Stimulus } &2.95 (0.93)\\
  \hline
    \raggedright{Both Audio and Visual } &3.10 (1.25)\\
  \hline
    \raggedright{Need Training } &3.95 (1.01)\\
  \hline
    \end{tabular}% For example,  
  \label{tab:relaysus}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%




















==> relay-user-v2.tex <==
%\section{Usability}
%
%\label{sec:usability}

In this section, we report on a user study of the reaction time relay attack
experiment presented previously in Section \ref{sec:relay-exp}.  We present the study design, goals, and
testing process, as well as study results.

\subsubsection{Study Design, Goals and Process}

In the relay attack study, users were given the task to play the games through
the interface which we developed (described in Section
\ref{sec:relay-implementation}). 
%The clicks on this interface were replicated on the online game version. 
The study comprised of 20 participants, primarily young undergraduate and
graduate students from Computer Science. This sample represents a near ideal
scenario for an attacker, given that young people typically have fast reaction
times \cite{kosinski}, which may increase the likelihood of the success of the
relay attack. The demographics of the participants are shown in
Table~\ref{tab:demographics-interviews} of the appendix. The study design was
similar to the one used in our usability study (Section \ref{sec:usability}).
It comprised of three phases.  The \textit{pre-study phase} involved
registering and briefly explaining the participants about the protocols of the
study.  In particular, the participants were shown ``consent information,''
which they had to agree before proceeding with the study.  This was followed by
collecting participant demographics and then the participants playing the games
via our interface.  
%This \textit{actual study phase} attempted to mimic a realistic captcha
%scenario which typically involves filling out a form followed by solving
%captcha.  To avoid explicit priming, however, we did not mention that the
%study is about captcha or security.  The final,
The participants were told to perform at their best in playing the games.
\textit{post-study phase} required the participants to respond to a few
questions about their experience and feedback on the games they played as part
of the interface. This included the Simple Usability Scale (SUS) \cite{sus}
questions and some additional questions regarding the usability of games.

%The scenario given for study required users to evaluate a new interface for
%registering for a website followed by playing 20 games. 
During the study, each participant was asked to play the relay versions corresponding to each the
20 variations of the four DCG captcha categories (described previously in Section \ref{sec:design}.
% implemented as discussed in
%Section \ref{sec:design}.  
%For each game category, these variations involve different parameters, i.e., object speed and number of objects per game.
%, affect
%the DCG captcha solving capability of the users. 
The order of the games
presented to the participants were counter-balanced for learning effects using
the Latin Square design (a 20 x 20 Latin Square was used).
%These were presented to each participant using Latin square methodology.  We
%were not required to go through an IRB approval process before conducting the
%experiments. However, authors of this paper have previously been involved in
%studies with U.S. Institutional Review Board (IRB) approvals, and have applied
%similar practices in this study.  


This relay attack study was conducted to answer and evaluate the following:
\begin{enumerate}
\vspace{-2mm}
\item {\textit{Efficiency}: time taken to complete the games (and succeeding at the relay attack}.
\vspace{-2mm}
\item {\textit{Robustness}: likelihood of not completing the game (relay attack failure) as well as the likelihood of incorrect drag and drop
attempts.}
\vspace{-2mm}
\item {\textit{User Experience}: quantitative SUS ratings and qualitative feedback from the participants about the game interface.}
\vspace{-2mm}
\item \textit{Effect of Game Parameters}: the effect of the number of object and objects speeds on completion time and error rates.
\vspace{-2mm}
\item  {\textit{Reaction time}: Time delay between the presentation of the stimulus and the response from the participant. This is a crucial metric for the feasibility of the attack. If reaction time is large, the likelihood of relay attack success will be low.}
%Time lapse between when clicks, till the game finishes or is timed out. We also Compare these solving rates to human solving the game in a realistic scenario (as in the user study)}
\vspace{-2mm}
\end{enumerate}

Another important goal of the relay study was to compare its performance with
that of the usability study. If the two differ significantly, the presence of
the relay attack can be easily detected based on this difference.
%Our study was conducted in a variety of campus venues including: student
%laboratories, cafes, student dorms/apartments, classrooms, ofÞce spaces and
%outdoor terraces .  After giving a brief overview of our study goals, we asked
%the participants to Þll out the background questionnaire to collect
%demographic information. This followed by a series 20 games to be played by
%the participants.Each user was asked to follow on-screen instructions in
%completing each task and was given a compensation of INR 75 for participating
%in the study.  

For each tested game, completion times, errors, actions and the playcount,
i.e., number of attempts made to successfully complete the games were
established, and automatically logged by the our web-interface software. In
addition, we maintained ``local logs'' of the clicks made by the participants
on the our game interface to measure the reaction timings.

\subsubsection{Study Results}

We present various mechanical data, i.e., time to completion and error rates
as part of the relay attack study. We further analyze the local logs for the reaction
time analysis.
%We nalize our interpretations by looking at all measures combined.

%\begin {itemize}


%% NS: Need to interpret these
\smallskip \noindent {\bf Completion Time and Error Rates}: Table
\ref{tab:relcaptcha} shows the time taken and error rates to play the games for
each game category by different participants. Unlike our usability study, many
game instances timed out, i.e., the participants were not able to complete
these game instances within the time out of 60 seconds.  In this light, we
report two types of timings: (1) \textit{successful time}, which is the time only
corresponding to the games that the participants were able to complete
successfully within the time out, and (2) \textit{overall time}, which is the
time corresponding to both the games instances completed successfully within the
time out and those which timed out (in which case we consider the timing to be
60 seconds).\footnote{The actual overall time will actually be higher.} 

Clearly, all games turned out to be quite slow, and much slower than that of
the usability study where the games lasted for less than 10 seconds on an
average (Section \ref{sec:usability}).  We found that users took maximum time
to solve the Animals game with an average overall time of 46.50 seconds (this
game was also the slowest in our usability study), whereas the other games took
comparably less, but similar amount of time. Similar to the usability study, this might have
been due to the increased semantic load in this game due to the presence of
three target objects.  As far as errors, we observed that the error rates were
the highest for the Animals game (40\%), and the least for the Shapes games
(0.09\%) 
%although the corresponding per click error rates were high (56\%). 
The
Ships and Parking games had comparable overall error rates between 20-30\%.
% but
%the Ships game per click error rate was the lowest (17\%). 
We analyzed and further compared the successful time for different game categories. The games showed
significantly different behavior from each other ($F=6.26, p=0.0007$). On
further analyzing the data, we found the following pairs of games to be 
%that the Parking and Ships games on
statistically different from each other: Parking and Ships ($p=0.0005$)
%. We also
%found the following pair of games to be significantly different form each other
Shapes and Ships ($p=0.013$), and Animals and all other games ($p<0.001$). 

%% NS: definitely needs to be understood and explained
To compare the error rates better, we investigated error rates per click, i.e.
for  each drag attempt whether the object being dragged was dropped at the
correct position or not. The error rate per click was the least for the Ships
game (0.17). 
%This is less than Shapes  game as the number of
%attempted clicks by the participants for this game were less. 

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time per game type}
        %\vspace{.2cm}
    \begin{tabular}{|p{1cm}|p{1.9cm}|p{1.5cm}|p{1cm}|p{.8cm}|}

   \hline
{\bf Game Type} &  \bf Overall Time (sec)& \bf Successful time &\bf Error Rate &\bf Error Rate Per click   \\
&  \textit{mean (std dev)}& \textit{mean (std dev)}&\textit{mean}& \textit{mean}   \\
 \hline
 \hline
    \raggedright{Ships} &30.92 (5.91) & 22.25 (5.04) & 0.26  &0.17 \\
 \hline
  \raggedright{Animals} &46.51 (5.05)&37.93 (4.91) & 0.40  &0.65  \\
\hline
  \raggedright{Parking} &28.16 (7.36) &20.45 (5.04) & 0.22  & 0.66  \\
  \hline
  \raggedright{Shapes} &26.19 (1.59)  &22.94 (1.74) &0.09 &  0.56 \\
\hline 
    \end{tabular}
  \label{tab:relcaptcha}
\end{center} 
}}
\vspace{-4mm}
\end{table}%






%The goal of our usability study was to evaluate and compare different DCG captcha games with
%respect to the following factors:

%\begin {enumerate}
%\item {Efficiency: time taken to complete each game}
%\item {Robustness: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts }
%\item {User Experience: quantitative SUS ratings and qualitative feedback from the participants.
%\end {enumerate}item 


\smallskip \noindent {\bf Effect of Object Speed}: Table \ref{tab:captchaspeed}
shows the performance of the games in terms of error rates and completion time
at different object speeds per game category.  
We can generally see that the timings increase as the speeds increase. The error rates per click
also follow the same pattern, although error rates do not exhibit such a behavior.
ANOVA tests on the timing measurements, however, 
did not show any significant impact of different speeds.
%presented to the participants ($F=2.90, p=0.06$). 


\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for various speed categories}
        %\vspace{.2cm}
     \begin{tabular}{|p{1cm}|p{1.9cm}|p{1.5cm}|p{1cm}|p{.8cm}|}
   \hline
{\bf Object Speed} &  \bf Overall Time (sec) &\bf Successful time & \bf Error Rate & \bf Error Rate Per click \\
&  \textit{mean (std dev)}& \textit{mean (std dev)}&\textit{mean}& \textit{mean}   \\
 \hline
 \hline
    \raggedright{10 FPS } &30.90 (9.03) &24.45 (0.08)&0.19 & 0.37 \\
 \hline
  \raggedright{20 FPS} &30.64 (8.93) &30.64 (0.09)&0.31 &0.43 \\
\hline
  \raggedright{40 FPS} &38.62 (10.34) &38.62 (0.10) &0.23  & 0.68 \\
  \hline
    \end{tabular}
  \label{tab:captchaspeed}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Effect of Number of Objects}: Another aspect of the
usability analysis included testing the effect of increase in the number of
objects (noise / incorrect answer objects) on the overall game performance.
Table \ref{tab:captchaobject} summarizes the error rates and time with
different number of objects.

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different number of objects.}
        %\vspace{.2cm}
    \begin{tabular}{|p{1cm}|p{1.9cm}|p{1.5cm}|p{1cm}|p{.8cm}|}
   \hline
{\bf Number of Objects} &  \bf Overall Time (sec) &\bf Successful time & \bf Error Rate & \bf Error Rate Per click \\
&  \textit{mean (std dev)}& \textit{mean (std dev)}&\textit{mean}& \textit{mean}   \\
 \hline
 \hline
    \raggedright{6} & 27.13 (10.40) &20.19 (0.05) &0.21 & 0.43\\
 \hline
  \raggedright{5} & 32.58 (8.64) &23.27 (0.08) &0.30  & 0.51  \\
\hline
  \raggedright{4} & 30.64 (8.93) &24.32 (0.09) &0.24 & 0.54  \\
  \hline 
    \end{tabular}
  \label{tab:captchaobject}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Reaction Time}:
%
%In this section, we discuss the reaction time i.e. time taken by the
%participants for each click on the objects. 
We now analyze the reaction time corresponding to different games during the relay attack experiments.
The averaged results are summarized in Table \ref{tab:relay1}.
We can see that the average reaction time for all game categories was 
more than 2 seconds and the least for
the Shapes game (2.17 seconds). The reaction
time did not change drastically across different game categories. This can be used to infer
that various games contributed same load on the users' reflexes.
Using the ANOVA test, we did however find
significant difference between the reaction time of the four games ($F=13.19,
p<0.01$). On further analyses using paired t-tests,
we found that there was a significant difference between the Animals
and Parking games ($p<0.01$).
 
Looking at Tables \ref{tab:relay2} and \ref{tab:relay3}, we did not find any
drastic differences in the reactions timings with respect to the number of
objects and speed. The reaction time was least for 10 FPS games (2.22 sec).
For the number of objects, surprisingly the reaction time was the least for
games with 6 objects. This can be because more number of objects likely
encouraged the users to click faster. ANOVA test did not indicate any
significant difference in the reaction timings for different speeds ($p=0.06$)
and number of objects ($p=0.4$).

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Reaction time for per game type}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Game Type} &  \bf Reaction Time (sec) \\
 \hline
 \hline
    \raggedright{Ships} &2.27 (0.34)\\
 \hline
  \raggedright{Animals} & 2.58 (0.35)\\
\hline
  \raggedright{Parking} & 2.5 (0.51) \\
  \hline
  \raggedright{Shapes} &2.17 (0.2)\\
\hline 
    \end{tabular}% For example,  
  \label{tab:relay1}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Completion time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Object Speed} &  \bf Reaction Time (sec) \\
 \hline
 \hline
    \raggedright{10 FPS } &2.22	(0.38)\\
 \hline
  \raggedright{20 FPS } & 2.36 (0.49)\\
\hline
  \raggedright{40 FPS } &2.35 (0.07)  \\
  \hline
    \end{tabular}% For example,  
  \label{tab:relay2}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Completion time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Number of Objects} &  \bf Reaction Time (sec) \\
 \hline
 \hline
    \raggedright{ 6 objects / game } & 2.11 (0.12)\\
 \hline
  \raggedright{ 5 objects / game }&2.82 (0.33)\\
\hline
  \raggedright{ 4 objects / game } &2.36 (0.49)  \\
  \hline
    \end{tabular}% For example,  
  \label{tab:relay3}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf User Experience}:
%
%To understand better the feasibility of human using interfaces (as the one we
%developed for the relay study) for relay attack, we conducted a post survey.
%The survey asked the participants to share their experiences while playing the
%games. 
We now consider the data collected via direct user responses during the
post-study phase.  The average SUS score from the study came out to be only
49.88 (std dev = xxx). This is rather low given that average scores for
commerical usable systems range from 60-70 \cite{susmean}, and suggests a poor
usability of the system. This means that it would be difficult for human users
to perform well at the relay attack tasks and implies that launching relay
attacks against DCG captcha can be quite challenging for an attacker.

%We asked participants few likert (scale: 1 -  5) questions about their feedback
%on the usability of the games. Various aspects of this included - `` if the
%games were visually attractive'', `` Were the games pleasurable'' etc.  Forty
%five percent participants felt the games to be visually attractive and 24\%
%said that it was pleasurable to play the games. 

%This number depicts high possibility of making such interfaces more usable for
%relay attacks and also can be thought of as an indicator of humans being able
%to use such interfaces for relay attack. 
The Table~\ref{tab:relaysus} shows the Likert scores for the visual appeal and
pleasurability of the games. Although the former average ratings are
reasonable (more that 3), the latter ratings are low; clearly the participants
did not find the games to be very pleasurable.  In our games, we made use of
visual and audio stimuli to which the users had to respond.  In order to
understand what type of stimulus worked best for the participants, we asked
them to what extent the audio, visual or both stimuli together was useful as an
indicator to respond fastest to the game.  These ratings are depicted in
Table~\ref{tab:relaysus}.  The responses were on average in favor of the visual
stimulus, followed by the two stimuli together, and finally the audio stimulus.
35\% participants found audio stimulus and visual stimulus to be sufficient
whereas 45\% participants agreed or strongly agreed with the statement that
both visual and audio stimulus are necessary to play the game.  We further
performed the ANOVA test and found a variance ($F=0.64, p=0.52$) for the three,
visual, audio and both stimulus, indicating no significant difference between
he three stimuli. Finally, and perhaps more importantly, 80\% of the
participants felt that training will help them play the games better with an
average score of 3.95. This beholds some promise for an attacker to launch
successful relay attack against DCG captchas by means of prior training given
to the human solvers.

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Completion time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Features} &  \bf Avg. Score\\
 \hline
 \hline
    \raggedright{Visually Attractive} & 3.20 (0.92)\\
 \hline
  \raggedright{Pleasurable } & 2.85 (0.99)\\
\hline
  \raggedright{Visual Stimulus } &3.20 (1.17)\\
  \hline
   \raggedright{Audio Stimulus } &2.95 (0.93)\\
  \hline
    \raggedright{Both Audio and Visual } &3.10 (1.25)\\
  \hline
    \raggedright{Need Training } &3.95 (1.01)\\
  \hline
    \end{tabular}% For example,  
  \label{tab:relaysus}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%




\smallskip \noindent {\bf Summary of Analysis}: All of our analyses above
suggest that perpetrating a successful relay attack against the DCG captcha
pose significant challenges. For the attack to succeed, the human-solver needs
to perform a reaction time task (average reaction time is more than 2 seconds),
which, except for the Shapes game, takes significantly longer amount of time
(more than about 30 seconds on average), is significantly more error prone
(error rates more than 20\%), and much harder for the users (average SUS less
than 50) when compared to directly playing the games in the honest setting. The human-solver
performance may be improved with training, but this may increase the economical
costs for the attacker.
















==> tt <==
This is pdfTeX, Version 3.1415926-2.3-1.40.12 (MiKTeX 2.9 64-bit)
entering extended mode
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\main.tex"
LaTeX2e <2011/06/27>
Babel <v3.8m> and hyphenation patterns for english, afrikaans, ancientgreek, ar
abic, armenian, assamese, basque, bengali, bokmal, bulgarian, catalan, coptic, 
croatian, czech, danish, dutch, esperanto, estonian, farsi, finnish, french, ga
lician, german, german-x-2009-06-19, greek, gujarati, hindi, hungarian, iceland
ic, indonesian, interlingua, irish, italian, kannada, kurmanji, lao, latin, lat
vian, lithuanian, malayalam, marathi, mongolian, mongolianlmc, monogreek, ngerm
an, ngerman-x-2009-06-19, nynorsk, oriya, panjabi, pinyin, polish, portuguese, 
romanian, russian, sanskrit, serbian, slovak, slovenian, spanish, swedish, swis
sgerman, tamil, telugu, turkish, turkmen, ukenglish, ukrainian, uppersorbian, u
senglishmax, welsh, loaded.
("C:\Program Files\MiKTeX 2.9\tex\latex\base\article.cls"
Document Class: article 2007/10/19 v1.4h Standard LaTeX document class
("C:\Program Files\MiKTeX 2.9\tex\latex\base\size10.clo"))
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xy.sty"
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xy.tex" Bootstrap'ing:
catcodes, docmode, ("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xyrecat.tex"
) ("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xyidioms.tex")

 Xy-pic version 3.8.6 <2011/05/27>
 Copyright (c) 1991-2011 by Kristoffer H. Rose <krisrose@tug.org>
 Xy-pic is free software: see the User's Guide for details.

Loading kernel: messages; fonts; allocations: state, direction,
utility macros; pictures: \xy, positions, objects, decorations;
kernel objects: directionals, circles, text; options; algorithms: directions,
edges, connections;  Xy-pic loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\ifpdf.sty")
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xyall.tex"
 Xy-pic option: All features v.3.8
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xycurve.tex"
 Xy-pic option: Curve and Spline extension v.3.12 curve, circles, loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xyframe.tex"
 Xy-pic option: Frame and Bracket extension v.3.13 loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xycmtip.tex"
 Xy-pic option: Computer Modern tip extension v.3.7
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xytips.tex"
 Xy-pic option: More Tips extension v.3.9 loaded) loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xyline.tex"
 Xy-pic option: Line styles extension v.3.10 loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xyrotate.tex"
 Xy-pic option: Rotate and Scale extension v.3.8 loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xycolor.tex"
 Xy-pic option: Colour extension v.3.11 loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xymatrix.tex"
 Xy-pic option: Matrix feature v.3.14 loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xyarrow.tex"
 Xy-pic option: Arrow and Path feature v.3.9 path, \ar, loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xygraph.tex"
 Xy-pic option: Graph feature v.3.11 loaded) loaded)
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xypdf.tex"
 Xy-pic option: PDF driver v.1.7 Xy-pic pdf driver: `color' extension support
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xypdf-co.tex" loaded)
Xy-pic pdf driver: `curve' extension support
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xypdf-cu.tex" loaded)
Xy-pic pdf driver: `frame' extension support
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xypdf-fr.tex" loaded)
Xy-pic pdf driver: `line' extension support
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xypdf-li.tex" loaded)
Xy-pic pdf driver: `rotate' extension support
("C:\Program Files\MiKTeX 2.9\tex\generic\xypic\xypdf-ro.tex" loaded) loaded))
("C:\Program Files\MiKTeX 2.9\tex\latex\floatflt\floatflt.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\amsfonts.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\ams\math\amscd.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\ams\math\amsgen.sty"))
("C:\Program Files\MiKTeX 2.9\tex\latex\ams\math\amsmath.sty"
For additional information on amsmath, use the `?' option.
("C:\Program Files\MiKTeX 2.9\tex\latex\ams\math\amstext.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\ams\math\amsbsy.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\ams\math\amsopn.sty"))
("C:\Program Files\MiKTeX 2.9\tex\latex\subfigure\subfigure.sty"
****************************************
* Local config file subfigure.cfg used *
****************************************
("C:\Program Files\MiKTeX 2.9\tex\latex\subfigure\subfigure.cfg"))
("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\graphicx.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\keyval.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\graphics.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\graphics\trig.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\00miktex\graphics.cfg")
("C:\Program Files\MiKTeX 2.9\tex\latex\pdftex-def\pdftex.def"
("C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\infwarerr.sty")
("C:\Program Files\MiKTeX 2.9\tex\generic\oberdiek\ltxcmds.sty"))))
("C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\times.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\breakurl\breakurl.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\xkeyval\xkeyval.sty"
("C:\Program Files\MiKTeX 2.9\tex\generic\xkeyval\xkeyval.tex"))

Package breakurl Warning: You are using breakurl while processing via pdflatex.

(breakurl)                \burl will be just a synonym of \url.
(breakurl)                 on input line 47.

) ("C:\Program Files\MiKTeX 2.9\tex\latex\ltxmisc\url.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\preprint\fullpage.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\boxedminipage\boxedminipage.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\base\ifthen.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\setspace\setspace.sty"
Package: `setspace' 6.7 <2000/12/01>
) ("C:\Program Files\MiKTeX 2.9\tex\latex\tools\xspace.sty")
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\usenix.sty
" ("C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\mathptmx.sty"))
("C:\Program Files\MiKTeX 2.9\tex\latex\titlesec\titlesec.sty")
("C:\Program Files\MiKTeX 2.9\tex\latex\caption\caption.sty"
("C:\Program Files\MiKTeX 2.9\tex\latex\caption\caption3.sty"))
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\main.aux"

LaTeX Warning: Label `tab:demographics-interviews' multiply defined.

) ("C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\ot1ptm.fd")
("C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\ot1ztmcm.fd")
("C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\omlztmcm.fd")
("C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\omsztmcm.fd")
("C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\omxztmcm.fd")
("C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\umsa.fd")
("C:\Program Files\MiKTeX 2.9\tex\latex\amsfonts\umsb.fd")
("C:\Program Files\MiKTeX 2.9\tex\context\base\supp-pdf.mkii"
[Loading MPS to PDF converter (version 2006.09.02).]
) ("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\intro.te
x"
Underfull \hbox (badness 1158) in paragraph at lines 25--35
[]\OT1/ptm/m/n/10 Unfortunately, ex-ist-ing captcha tech-nol-ogy suf-fers
<figs/face.pdf, id=1, 454.69875pt x 205.76875pt> <use figs/face.pdf> [1{C:/Prog
ramData/MiKTeX/2.9/pdftex/config/pdftex.map} <C:/Users/saxena/Desktop/Backup100
82011/Desktop/Papers/Game CAPTCHA/figs/face.pdf>]
Underfull \hbox (badness 2261) in paragraph at lines 115--116
[]\OT1/ptm/m/n/10 We de-sign and im-ple-ment a sam-ple of DCG

Underfull \hbox (badness 1057) in paragraph at lines 127--129
[]\OT1/ptm/m/n/10 We con-duct a us-abil-ity study of DCG captcha

Underfull \hbox (badness 1097) in paragraph at lines 127--129
\OT1/ptm/m/n/10 and an-a-lyze its fea-si-bil-ity in terms of time-to-
)
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\background
.tex" [2] <figs/ships.jpg, id=23, 361.35pt x 130.4875pt> <use figs/ships.jpg>
<figs/shapes.jpg, id=24, 361.35pt x 130.4875pt> <use figs/shapes.jpg>
<figs/boat-parking.jpg, id=25, 361.35pt x 130.4875pt>
<use figs/boat-parking.jpg>
<figs/feed-animals.jpg, id=26, 361.35pt x 130.4875pt>
<use figs/feed-animals.jpg> [3])
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\design.tex
" [4 <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/s
hips.jpg> <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/f
igs/shapes.jpg> <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAP
TCHA/figs/boat-parking.jpg> <C:/Users/saxena/Desktop/Backup10082011/Desktop/Pap
ers/Game CAPTCHA/figs/feed-animals.jpg>])
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\usability.
tex"
Underfull \hbox (badness 10000) in paragraph at lines 122--122
[]\OT1/ptm/b/n/8 Completion

Underfull \hbox (badness 10000) in paragraph at lines 122--123
[]\OT1/ptm/b/n/8 Error
[5]
Underfull \hbox (badness 10000) in paragraph at lines 206--206
[]\OT1/ptm/b/n/8 Completion

Underfull \hbox (badness 10000) in paragraph at lines 206--207
[]\OT1/ptm/b/n/8 Error

Underfull \hbox (badness 10000) in paragraph at lines 244--244
[]\OT1/ptm/b/n/8 Completion

Underfull \hbox (badness 10000) in paragraph at lines 244--245
[]\OT1/ptm/b/n/8 Error
[6])
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\computatio
nal.tex" <figs/attackdiagram.pdf, id=42, 706.24344pt x 372.45325pt>
<use figs/attackdiagram.pdf>
("C:\Program Files\MiKTeX 2.9\tex\latex\psnfss\ot1pcr.fd") [7]
Underfull \hbox (badness 1931) in paragraph at lines 208--216
[]\OT1/ptm/m/n/10 Each learned back-ground im-age is saved in the
<figs/TEST.pdf, id=47, 722.7pt x 542.025pt> <use figs/TEST.pdf>
<figs/FIG-3.pdf, id=48, 722.7pt x 542.025pt> <use figs/FIG-3.pdf> [8 <C:/Users/
saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/attackdiagram.pd
f> <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/TES
T.pdf>] <figs/mbr.pdf, id=119, 722.7pt x 542.025pt> <use figs/mbr.pdf>
<figs/FIG-4.pdf, id=120, 722.7pt x 542.025pt> <use figs/FIG-4.pdf>

LaTeX Warning: `h' float specifier changed to `ht'.

<figs/FIG-5.pdf, id=121, 722.7pt x 542.025pt> <use figs/FIG-5.pdf> [9 <C:/Users
/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/FIG-3.pdf> <C:/
Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/mbr.pdf> <
C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/FIG-4.p
df>] [10 <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/fi
gs/FIG-5.pdf>]
Underfull \hbox (badness 1331) in paragraph at lines 693--708
\OT1/ptm/m/it/10 Attacking: \OT1/ptm/m/n/10 Dur-ing at-tack-ing, there is a tim
e lapse
) ("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\relay.te
x" [11] <figs/relay.pdf, id=205, 722.7pt x 542.025pt> <use figs/relay.pdf>

LaTeX Warning: `h' float specifier changed to `ht'.

[12 <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/re
lay.pdf>]
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\relay-user
.tex"

LaTeX Warning: Reference `tab:relay-demographics-interviews' on page 13 undefin
ed on input line 21.

[13]
Underfull \hbox (badness 10000) in paragraph at lines 165--165
[]\OT1/ptm/b/n/8 Game

Underfull \hbox (badness 10000) in paragraph at lines 165--165
[]\OT1/ptm/b/n/8 Overall Time

Underfull \hbox (badness 10000) in paragraph at lines 165--165
[]\OT1/ptm/b/n/8 Successful

Underfull \hbox (badness 10000) in paragraph at lines 165--165
[]\OT1/ptm/b/n/8 Error

Underfull \hbox (badness 10000) in paragraph at lines 165--166
[]\OT1/ptm/b/n/8 Error

Underfull \hbox (badness 10000) in paragraph at lines 165--166
\OT1/ptm/b/n/8 Rate

Underfull \hbox (badness 10000) in paragraph at lines 165--166
\OT1/ptm/b/n/8 Per

Underfull \hbox (badness 10000) in paragraph at lines 166--166
[]\OT1/ptm/m/it/8 mean (std

Overfull \hbox (10.5632pt too wide) in paragraph at lines 162--179
 [] 

Underfull \hbox (badness 10000) in paragraph at lines 217--217
[]\OT1/ptm/b/n/8 Object

Underfull \hbox (badness 10000) in paragraph at lines 217--217
[]\OT1/ptm/b/n/8 Overall Time

Underfull \hbox (badness 10000) in paragraph at lines 217--217
[]\OT1/ptm/b/n/8 Successful

Underfull \hbox (badness 10000) in paragraph at lines 217--217
[]\OT1/ptm/b/n/8 Error

Underfull \hbox (badness 10000) in paragraph at lines 217--218
[]\OT1/ptm/b/n/8 Error

Underfull \hbox (badness 10000) in paragraph at lines 217--218
\OT1/ptm/b/n/8 Rate

Underfull \hbox (badness 10000) in paragraph at lines 217--218
\OT1/ptm/b/n/8 Per

Underfull \hbox (badness 10000) in paragraph at lines 218--218
[]\OT1/ptm/m/it/8 mean (std

Overfull \hbox (10.5632pt too wide) in paragraph at lines 215--229
 [] 
[14]
Underfull \hbox (badness 10000) in paragraph at lines 248--248
[]\OT1/ptm/b/n/8 Number

Underfull \hbox (badness 10000) in paragraph at lines 248--248
\OT1/ptm/b/n/8 of

Underfull \hbox (badness 10000) in paragraph at lines 248--248
[]\OT1/ptm/b/n/8 Overall Time

Underfull \hbox (badness 10000) in paragraph at lines 248--248
[]\OT1/ptm/b/n/8 Successful

Underfull \hbox (badness 10000) in paragraph at lines 248--248
[]\OT1/ptm/b/n/8 Error

Underfull \hbox (badness 10000) in paragraph at lines 248--249
[]\OT1/ptm/b/n/8 Error

Underfull \hbox (badness 10000) in paragraph at lines 248--249
\OT1/ptm/b/n/8 Rate

Underfull \hbox (badness 10000) in paragraph at lines 248--249
\OT1/ptm/b/n/8 Per

Underfull \hbox (badness 10000) in paragraph at lines 249--249
[]\OT1/ptm/m/it/8 mean (std

Overfull \hbox (10.5632pt too wide) in paragraph at lines 246--260
 [] 

Underfull \hbox (badness 10000) in paragraph at lines 322--322
[]\OT1/ptm/b/n/8 Game

Underfull \hbox (badness 10000) in paragraph at lines 322--324
[]\OT1/ptm/b/n/8 Reaction Time

Underfull \hbox (badness 10000) in paragraph at lines 322--324
\OT1/ptm/b/n/8 Cor-rect Clicks

Underfull \hbox (badness 10000) in paragraph at lines 351--351
[]\OT1/ptm/b/n/8 Object

Underfull \hbox (badness 10000) in paragraph at lines 351--353
[]\OT1/ptm/b/n/8 Reaction Time

Underfull \hbox (badness 10000) in paragraph at lines 351--353
\OT1/ptm/b/n/8 Cor-rect Clicks

Underfull \hbox (badness 10000) in paragraph at lines 378--378
[]\OT1/ptm/b/n/8 Number

Underfull \hbox (badness 10000) in paragraph at lines 378--379
[]\OT1/ptm/b/n/8 Reaction Time

Underfull \hbox (badness 10000) in paragraph at lines 378--379
\OT1/ptm/b/n/8 Cor-rect Clicks
[15]))
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\discussion
.tex")
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\related.te
x" <figs/captcha-taxonomy.pdf, id=254, 722.7pt x 542.025pt>
<use figs/captcha-taxonomy.pdf>
Underfull \hbox (badness 1264) in paragraph at lines 19--39
[]\OT1/ptm/m/n/10 Character-recognition (CR) captchas are the most

Underfull \hbox (badness 6268) in paragraph at lines 49--56
\OT1/ptm/m/n/10 ques-tions, and se-man-tic tasks re-lated to im-ages

Underfull \hbox (badness 2617) in paragraph at lines 67--77
[]\OT1/ptm/m/n/10 The captcha lit-er-a-ture in-cludes work on ro-bust-
)
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\conclusion
.tex")
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\main.bbl"
Underfull \hbox (badness 10000) in paragraph at lines 4--7
[]\OT1/ptm/m/n/8 Cracking the arey-ouahu-man captcha.  $\OT1/pcr/m/n/8 http : /
 /

Underfull \hbox (badness 10000) in paragraph at lines 4--7
\OT1/pcr/m/n/8 spamtech . co . uk / software / bots / cracking -[] the -[]
[16 <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/ca
ptcha-taxonomy.pdf>]
Underfull \hbox (badness 10000) in paragraph at lines 72--76
\OT1/pcr/m/n/8 net / 2004 / 01 / 27 / solving _ and _ creating . html$\OT1/ptm/
m/n/8 ,

Underfull \hbox (badness 1122) in paragraph at lines 114--117
[]\OT1/ptm/m/n/8 Dancho Danchev.  In-side in-dias captcha solv-ing econ-omy.

Underfull \hbox (badness 2941) in paragraph at lines 114--117
\OT1/ptm/m/n/8 Avail-able at: $\OT1/pcr/m/n/8 http : / / blogs . zdnet . com / 
security /

Underfull \hbox (badness 10000) in paragraph at lines 149--154
[]\OT1/ptm/m/n/8 G. Keizer.  Spam-mers' Bot Cracks Mi-crosoft's

Underfull \hbox (badness 1448) in paragraph at lines 149--154
\OT1/ptm/m/n/8 CAPTCHA .  In \OT1/ptm/m/it/8 Com-puter World\OT1/ptm/m/n/8 , Av
ail-able at: $\OT1/pcr/m/n/8 http :

Underfull \hbox (badness 10000) in paragraph at lines 149--154
\OT1/pcr/m/n/8 / / www . computerworld . com / s / article / 9061558 /

Underfull \hbox (badness 10000) in paragraph at lines 149--154
\OT1/pcr/m/n/8 Spammers _ bot _ cracks _ Microsoft _ s _ CAPTCHA_$\OT1/ptm/m/n/
8 ,

Underfull \hbox (badness 10000) in paragraph at lines 194--198
\OT1/pcr/m/n/8 http : / / www . kloover . com / 2008 / 05 / 12 / breaking -[]

Underfull \hbox (badness 1874) in paragraph at lines 245--248
[]\OT1/ptm/m/n/8 NuCaptcha.  Nu-captcha: Adap-tive captcha au-then-ti-ca-tion.

Underfull \hbox (badness 10000) in paragraph at lines 250--254
\OT1/pcr/m/n/8 6352 / CAPTCHA -[] Can -[] Kill -[] Your -[] Conversion -[]

Underfull \hbox (badness 10000) in paragraph at lines 265--270
\OT1/pcr/m/n/8 http : / / www . prnewswire . com / news -[] releases /

Underfull \hbox (badness 10000) in paragraph at lines 265--270
\OT1/pcr/m/n/8 are -[] you -[] a -[] humans -[] user -[] friendly -[] game -[]

Underfull \hbox (badness 10000) in paragraph at lines 265--270
\OT1/pcr/m/n/8 based -[] security -[] solution -[] aims -[] to -[] replace -[]
[17])
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\appendix.t
ex" <figs/star.jpg, id=314, 361.35pt x 130.4875pt> <use figs/star.jpg>
<figs/cross.jpg, id=315, 361.35pt x 130.4875pt> <use figs/cross.jpg>
<figs/UI-start.png, id=316, 407.5225pt x 408.52625pt> <use figs/UI-start.png>
<figs/UI-next.png, id=317, 408.52625pt x 406.51875pt> <use figs/UI-next.png>
<figs/UI-new.png, id=318, 407.5225pt x 406.51875pt> <use figs/UI-new.png>)
[18 <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/figs/st
ar.jpg> <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game CAPTCHA/fig
s/cross.jpg>] [19 <C:/Users/saxena/Desktop/Backup10082011/Desktop/Papers/Game C
APTCHA/figs/UI-start.png> <C:/Users/saxena/Desktop/Backup10082011/Desktop/Paper
s/Game CAPTCHA/figs/UI-next.png> <C:/Users/saxena/Desktop/Backup10082011/Deskto
p/Papers/Game CAPTCHA/figs/UI-new.png>]
("C:\Users\saxena\Desktop\Backup10082011\Desktop\Papers\Game CAPTCHA\main.aux")

LaTeX Warning: There were undefined references.


LaTeX Warning: There were multiply-defined labels.

 )
(see the transcript file for additional information){C:/Program Files/MiKTeX 2.
9/fonts/enc/dvips/fontname/8r.enc}<C:/Program Files/MiKTeX 2.9/fonts/type1/publ
ic/amsfonts/cm/cmmi10.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/public/amsfo
nts/cm/cmr10.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/public/amsfonts/cm/cm
sy10.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/urw/courier/ucrr8a.pfb><C:/Pr
ogram Files/MiKTeX 2.9/fonts/type1/urw/times/utmb8a.pfb><C:/Program Files/MiKTe
X 2.9/fonts/type1/urw/times/utmbi8a.pfb><C:/Program Files/MiKTeX 2.9/fonts/type
1/urw/times/utmr8a.pfb><C:/Program Files/MiKTeX 2.9/fonts/type1/urw/times/utmri
8a.pfb>
Output written on main.pdf (19 pages, 1519175 bytes).
Transcript written on main.log.


==> usability-v0.tex <==
\section{Usability}
\label{sec:usability}

In this section, we report on a usability study of DCG captcha, including the
study design, goals, and testing process, as well as study results.

\subsection{Study Design, Goals and Testing Process}

Our study was undertaken by 40 participants. The corpus of participants
comprised primarily of undergraduate and graduate students from various
backgrounds. The demographics of the participants are shown in Table
\ref{tab:demographics-interviews}. The study was \textit{web-based} and
comprised of three phases. The \textit{pre-study phase} involved registering
and briefly explaining the participants about the protocols of the study.  In
particular, the participants were shown ``consent information,'' which they had
to agree before proceeding with the study.  This was followed by collecting
participant demographics and then the participants playing the different DCG
captcha games.  This \textit{actual study phase} attempted to mimic a realistic
captcha scenario which typically involves filling out a form followed by
solving captcha. To avoid explicit priming, however, we did not mention that
the study is about captcha or security, but rather indicated that it is about
assessing the usability of a web interface.  The final, \textit{post-study
phase} required the participants to respond to a few questions about their
experience and feedback on the games they played as part of the interface. This
included some questions on the usability of games and SUS. 

%The scenario given for study required users to evaluate a new interface for
%registering for a website followed by playing 20 games. 
During the acutual study phase, each participant was asked to play 20
variations of the four DCG captcha categories implemented as discussed in Section
\ref{sec:design}. 
These variations were aimed at understanding how different parameters, i.e., object speed and
number of objects per game, affect the DCG captcha solving capability of the users. 
The order of the games presented to the participants were
counter-balanced for learning effects using the Latin Square design (a 20 x 20
Latin Square was used).
%These were presented to each participant using Latin square methodology. 
%We were not required to go through an IRB approval process before conducting
%the experiments. However, authors of this paper have previously been involved
%in studies with U.S. Institutional Review Board (IRB) approvals, and have
%applied similar practices in this study.  

%\begin{table}[htdp]
%{\footnotesize{
%\caption{Demographics of the participants.}
%\begin{center}
%\small
%\begin{tabular}{|p{5cm}| r |}
%%\rowcolors {1}{orange!35 }{ }
%\hline
%\textbf{}& \textbf{N=40} \\
%\hline
%\hline
%%\textbf{Participants}& 16 & 20 \\
%%\hline
%%\hline
%\textbf{Gender} & \\
%\hline
% Male &7 \\
% \hline
%Female&9 \\
%\hline
% \hline
%\textbf{Age} & \\
%\hline
%
%less than 18 &0 \\
%\hline
%18 - 24 &3 \\
% \hline
% 25 - 35 &1 \\
%  \hline
%35 - 50  &4\\
%  \hline
%50 - 65  &4\\
% \hline
%  \hline
%\textbf{Education} & \\
%\hline 
%Highschool &3 \\
% \hline
%Bachelors  &8  \\
% \hline
%Masters &5 \\
%\hline
%Ph. D. & 8 \\
% \hline
%  \hline
%\textbf{Profession / field of study} & \\
%  \hline
%Computer Science & 3\\
%  \hline
%Engineering &6 \\
% \hline
%Medicine & 7 \\
% \hline
% Science, Pharmaceuticals & 4\\
% \hline
%%Have a Webmail account & & \\
% Law &\\
% \hline
%Social sciences  & 8\\
%  \hline
% Others  & 8\\
%  \hline
%\end{tabular}
%\normalsize
%\end{center}
%\label{tab:demographics-interviews}
%}}
%\end{table}

The specific goal of our usability study was to evaluate and compare different DCG captcha games with
respect to the following factors:

\begin {enumerate}


\item {\textit{Efficiency}: time taken to complete each game}
\item {\textit{Robustness}: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts.}
\item {\textit{User Experience}: quantitative SUS ratings and qualitative feedback from the participants.}
\item \textit{Effect of Game Parameters}: the effect of the number of object and objects speeds on completion time and error rates

\end {enumerate}

%Our study was conducted in a variety of campus venues including: student
%laboratories, cafes, student dorms/apartments, classrooms, of�ce spaces and
%outdoor terraces .  After giving a brief overview of our study goals, we asked
%the participants to �ll out the background questionnaire to collect demographic
%information. This followed by a series 20 games to be played by the
%participants.Each user was asked to follow on-screen instructions in completing
%each task and was given a compensation of INR 75 for participating in the
%study.  
For each tested game, completion times, errors, actions and the playcount,
i.e., number of attempts made to successfully complete the games were
established, and automatically logged by the our web-interface software.

\subsection{Study Results}

We now provide the results from our usability study. We
first consider various mechanical data, i.e., time to completion and error
rates. Then, we analyze perceived qualitative aspects of the methods based on
collected user ratings. 
%We nalize our interpretations by looking at all
%measures combined.


%\begin {itemize}

\smallskip \noindent {\bf Completion Time}: Table \ref{tab:captchaeff} shows
the time taken to complete the games per game category. Clearly, all games
turned out to be quite fast, lasting for less than 10 seconds on an average
(this far lower than our time out of 1 second).  We also found that users took
maximum time to solve the Animals game with an average time of 9.25 seconds,
whereas the other games took almost half of this time.  This might have been
due to increased semantic load on the users to identify three target objects
and then match them with the corresponding answer objects. Moreover, we noticed
a significant decrease in the solving time (4.09 sec) when the target objects
were decreased to 2 (i.e., in the Shapes game), and the time was comparable to
games which had 1 target object in the challenge (the Ships game and the
Parking game). 

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Completion time for each captcha game category}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Game} &  \bf Completion Time (sec) \\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &4.94  \\
 \hline
  \raggedright{Feed the Animals} &9.25  \\
\hline
  \raggedright{Park the Boat} &4.53  \\
  \hline
  \raggedright{Match the Shapes} &5.16\\
\hline 
    \end{tabular}% For example,  
  \label{tab:captchaeff}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%


\smallskip \noindent {\bf Error Rates}:  An important result from our study is
that all the tested games yielded 100\% accuracy (overall error rate of 0\%).
In other words, none of the participant failed to complete any of the games
within the time out. This proves that DCG captchas can be highly robust in
practice.  

Next, we calculated the likelihood of exhibiting incorrect drag and drop
attempts. For example,  in the Animals game, an incorrect attempt would be to
feed the monkey with a flower instead of a banana.  We define the error rate in
this context as the number of incorrect objects (from the pool of probable
answer objects) dragged to the target area divided by the total of objects
dragged and dropped. The results are depicted in Table \ref{tab:captchaerror}.
Looking at the table, we observe that the Shape game yields the smallest error
rate with 6\% of incorrect attempts on an average for various speeds and number
of objects. This suggests that the visual matching task (as in the Shapes game)
is less error prone compared to the semantic matching task (as in the other
games).  The Shapes game error rate was marginally (by 1\%) lower than the
Ships game and the Animals game. The game challenge which seemed most difficult
for the participants to solve was the Parking game (10\% error rate). Since
this was an empty target game, with the target region and the object region
having the same background, the participants may have found it a little
difficult to perform the matching task.

\begin{table}[ht]
{\footnotesize{
 \begin{center} 
  \caption{Error  rate (incorrect attempts / total attempts) for each captcha game category.}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Game} &  \bf Error Rate (\%)\\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &6  \\
 \hline
  \raggedright{Feed the Animals} &6  \\
\hline
  \raggedright{Park the Boat} &10  \\
  \hline
  \raggedright{Match the Shapes} &5\\
\hline 
    \end{tabular}
  \label{tab:captchaerror}
 \end{center} 
}}
\vspace{-4mm}
\end{table}
%The goal of our usability study was to evaluate and compare different DCG captcha games with
%respect to the following factors:

%\begin {enumerate}
%\item {Efficiency: time taken to complete each game}
%\item {Robustness: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts }
%\item {User Experience: quantitative SUS ratings and qualitative feedback from the participants.
%\end {enumerate}item 

\smallskip
\noindent {\bf User Experience:}


\smallskip \noindent {\bf Effect of Object Speed}: Table \ref{tab:captchaspeed}
shows the performance of the games in terms of error rates and completion time
at different object speeds per game category.  To evaluate the affect of speed on performance of
the participants, we found the correlation between error rates and time taken
to solve various game at different speed levels. The correlation came to be
-0.5 showing that participants took almost same time irrespective of the error.
We also found that maximum number of errors were committed at 40 FPS speed
which demonstrate some level of difficulty for users to be able to solve the
games at faster speeds.



\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for various speed categories}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Object Speed} &  \bf Error Rate (\%)& \bf Completion Time (sec) \\
 \hline
 \hline
    \raggedright{10 FPS } &5 &6.14 \\
 \hline
  \raggedright{20 FPS} &6 &5.31  \\
\hline
  \raggedright{40 FPS} &8 &6.13  \\
  \hline
    \end{tabular}
  \label{tab:captchaspeed}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Effect of Number of Objects}: Another aspect of the
usability analysis included testing the effect of increase in the number of
objects (noise / incorrect answer objects) on the overall game performance.
Table \ref{tab:captchaobject} summarizes the error rates and time with
different number of objects.  We found a strong correlation (0.95) between the
number of objects and completion, whereas there was no significant effect of
number of objects on error rate with correlation value of 0.32.

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different number of objects.}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Number of Objects} &  \bf Error Rate (\%) & \bf Completion Time (sec) \\
 \hline
 \hline
    \raggedright{ 6 objects / game } &8 &6.63 \\
 \hline
  \raggedright{5 objects / game} &5 &5.61  \\
\hline
  \raggedright{4 objects / game} &7 & 5.33 \\
  \hline 
    \end{tabular}
  \label{tab:captchaobject}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Summary of Analysis:} Based on our analysis, we can
conclude that the DCG captcha categories tested in this work offer very good
usability, resulting in short completion times (less than 10 sec), very low
error rates (0\% per game completion, and less than 10\% per drag and drop
attempt), and high user ratings. We also find that increasing the object speed
and number of objects is likely to negatively affect the game performance, but
up to 6 objects and up to 40 FPS speed yield a high level of usability. 




==> usability-v1.tex <==
\section{Usability}
\label{sec:usability}

In this section, we report on a usability study of DCG captcha, including the
study design, goals, and testing process, as well as study results.

\subsection{Study Design, Goals and Testing Process}

Our study was undertaken by 40 participants. The corpus of participants
comprised primarily of undergraduate and graduate students from various
backgrounds. The demographics of the participants are shown in Table
\ref{tab:demographics-interviews}. The study was \textit{web-based} and
comprised of three phases. The \textit{pre-study phase} involved registering
and briefly explaining the participants about the protocols of the study.  In
particular, the participants were shown ``consent information,'' which they had
to agree before proceeding with the study.  This was followed by collecting
participant demographics and then the participants playing the different DCG
captcha games.  This \textit{actual study phase} attempted to mimic a realistic
captcha scenario which typically involves filling out a form followed by
solving captcha. To avoid explicit priming, however, we did not mention that
the study is about captcha or security, but rather indicated that it is about
assessing the usability of a web interface.  The final, \textit{post-study
phase} required the participants to respond to a few questions about their
experience and feedback on the games they played as part of the interface. This
included some questions on the usability of games and SUS. 

%The scenario given for study required users to evaluate a new interface for
%registering for a website followed by playing 20 games. 
During the acutual study phase, each participant was asked to play 20
variations of the four DCG captcha categories implemented as discussed in Section
\ref{sec:design}. 
These variations were aimed at understanding how different parameters, i.e., object speed and
number of objects per game, affect the DCG captcha solving capability of the users. 
The order of the games presented to the participants were
counter-balanced for learning effects using the Latin Square design (a 20 x 20
Latin Square was used).
%These were presented to each participant using Latin square methodology. 
%We were not required to go through an IRB approval process before conducting
%the experiments. However, authors of this paper have previously been involved
%in studies with U.S. Institutional Review Board (IRB) approvals, and have
%applied similar practices in this study.  

\begin{table}[htdp]
{\footnotesize{
\caption{Demographics of the participants.}
\begin{center}
\small
\begin{tabular}{|p{5cm}| r |}
%\rowcolors {1}{orange!35 }{ }
\hline
\textbf{}& \textbf{N=40} \\
\hline
\hline
%\textbf{Participants}& 16 & 20 \\
%\hline
%\hline
\textbf{Gender} & (\%) \\
\hline
 Male & 50\\
 \hline
Female& 50 \\
\hline
 \hline
\textbf{Age} & (\%) \\
\hline

less than 18 &0  \\
\hline
18 - 24 & 80 \\
 \hline
 25 - 35 & 20 \\
  \hline
35 - 50  & 0\\
  \hline
50 - 65  & 0\\
 \hline
  \hline
\textbf{Education} & (\%) \\
\hline 
Highschool & 45 \\
 \hline
Bachelors  & 27.5\\
 \hline
Masters & 22.5\\
\hline
Ph. D. & 5 \\
 \hline
  \hline
\textbf{Profession / field of study} & (\%) \\
  \hline
Computer Science & 60 \\
  \hline
Engineering & 5 \\
 \hline
Science, Pharmaceuticals & 10\\
 \hline
%Have a Webmail account & & \\
 Law & 2.5\\
 \hline
Journalism  & 2.5 \\
  \hline
Finance  & 2.5 \\
  \hline
Business  & 5 \\
  \hline
 Others  &12.5 \\
  \hline
\end{tabular}
\normalsize
\end{center}
\label{tab:demographics-interviews}
}}
\end{table}

The specific goal of our usability study was to evaluate and compare different DCG captcha games with
respect to the following factors:

\begin {enumerate}


\item {\textit{Efficiency}: time taken to complete each game}
\item {\textit{Robustness}: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts.}
\item {\textit{User Experience}: quantitative SUS ratings and qualitative feedback from the participants.}
\item \textit{Effect of Game Parameters}: the effect of the number of object and objects speeds on completion time and error rates

\end {enumerate}

%Our study was conducted in a variety of campus venues including: student
%laboratories, cafes, student dorms/apartments, classrooms, ofÞce spaces and
%outdoor terraces .  After giving a brief overview of our study goals, we asked
%the participants to Þll out the background questionnaire to collect demographic
%information. This followed by a series 20 games to be played by the
%participants.Each user was asked to follow on-screen instructions in completing
%each task and was given a compensation of INR 75 for participating in the
%study.  
For each tested game, completion times, errors, actions and the playcount,
i.e., number of attempts made to successfully complete the games were
established, and automatically logged by the our web-interface software.

\subsection{Study Results}

We now provide the results from our usability study. We
first consider various mechanical data, i.e., time to completion and error
rates. Then, we analyze perceived qualitative aspects of the methods based on
collected user ratings. 
%We nalize our interpretations by looking at all
%measures combined.


%\begin {itemize}

\smallskip \noindent {\bf Completion Time}: Table \ref{tab:captchaeff} shows
the time taken to complete the games per game category. Clearly, all games
turned out to be quite fast, lasting for less than 10 seconds on an average
(this far lower than our time out of 1 second).  We also found that users took
maximum time to solve the Animals game with an average time of 9.06 seconds,
whereas the other games took almost half of this time.  This might have been
due to increased semantic load on the users to identify three target objects
and then match them with the corresponding answer objects. Moreover, we noticed
a significant decrease in the solving time (3.83 sec) when the target objects
were decreased to 2 (i.e., in the Shapes game), and the time was comparable to
games which had 1 target object in the challenge (the Ships game and the
Parking game).  We found significant difference between all 4 categories of games (p$<$0.001), on solving time.  On analyzing further, we found significant difference between animal - boast parking games (p$<$0.001), ship - shape game ( p=0.0019), animal - ship game (p<0.001), animal - shape (p=0.00195) and parking - shape game (p=0.0005)

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different categories of games}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Game type} &  \bf Average Time (sec)& \bf Error Rate    \\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &4.74 (1.06) & 0.04 (0.02) \\
 \hline
  \raggedright{Feed the Animals} &9.06 (0.90)&0.05 (0.05)  \\
\hline
  \raggedright{Park the Boat} &4.37 (0.86) &0.09 (0.03)  \\
  \hline
  \raggedright{Match the Shapes} &5.23 (0.64)  &0.03 (0.02)\\
\hline 
    \end{tabular}
  \label{tab:captchaeff}
\end{center} 
}}
\vspace{-4mm}
\end{table}%


\smallskip \noindent {\bf Error Rates}:  An important result from our study is
that all the tested games yielded 100\% accuracy (overall error rate of 0\%).
In other words, none of the participant failed to complete any of the games
within the time out. This proves that DCG captchas can be highly robust in
practice.  

Next, we calculated the likelihood of exhibiting incorrect drag and drop
attempts. For example,  in the Animals game, an incorrect attempt would be to
feed the monkey with a flower instead of a banana.  We define the error rate in
this context as the number of incorrect objects (from the pool of probable
answer objects) dragged to the target area divided by the total of objects
dragged and dropped. The results are depicted in Table \ref{tab:captchaeff}.
Looking at the table, we observe that the Shape game yields the smallest error
rate with 0.03\% of incorrect attempts on an average for various speeds and number
of objects. This suggests that the visual matching task (as in the Shapes game)
is less error prone compared to the semantic matching task (as in the other
games). The game challenge which seemed most difficult
for the participants to solve was the Parking game (0.09). Since
this was an empty target game, with the target region and the object region
having the same background, the participants may have found it a little
difficult to perform the matching task.


%The goal of our usability study was to evaluate and compare different DCG captcha games with
%respect to the following factors:

%\begin {enumerate}
%\item {Efficiency: time taken to complete each game}
%\item {Robustness: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts }
%\item {User Experience: quantitative SUS ratings and qualitative feedback from the participants.
%\end {enumerate}item 


\smallskip \noindent {\bf Effect of Object Speed}: Table \ref{tab:captchaspeeduser}
shows the performance of the games in terms of error rates and completion time
at different object speeds per game category.  To evaluate the affect of speed on performance of
the participants, we found the correlation between error rates and time taken
to solve various game at different speed levels.
We also found that maximum number of errors were committed at 10 FPS speed
which demonstrate some level of difficulty for users to be able to solve the
games at lower speeds. There exists statistical difference between the three speeds on the time spent in solving the games (p=0.006).  We found using t-test that their existed statistical difference between the following pair of speeds in different game variants - 10FPS and 20FPS (p$<$0.001) and 20FPS - 40FPS (p=0.0004)



\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for various speed categories}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Object Speed} &  \bf Avg. Play Time (sec) & \bf  Error Rate\\
 \hline
 \hline
    \raggedright{10 FPS } &5.80 (2.14) &0.06 (0.06)  \\
 \hline
  \raggedright{20 FPS} &4.88(2.20) &0.05 (0.04)  \\
\hline
  \raggedright{40 FPS} &6.50 (2.81) &0.04 (0.01)  \\
  \hline
    \end{tabular}
  \label{tab:captchaspeeduser}
\end{center} 
}}
\vspace{-4mm}
\end{table}%


\smallskip \noindent {\bf Effect of Number of Objects}: Another aspect of the
usability analysis included testing the effect of increase in the number of
objects (noise / incorrect answer objects) on the overall game performance.
Table \ref{tab:captchaobjectuser} summarizes the error rates and time with
different number of objects.

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time for different number of objects.}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|}
   \hline
{\bf Number of Objects} &  \bf Error Rate (\%) & \bf Avg. Play Time (sec)\\
 \hline
 \hline
    \raggedright{ 6 objects / game } &6.52 (1.69) &0.06 (0.03) \\
 \hline
  \raggedright{5 objects / game} &5.34 (2.32) &0.05 (0.04) \\
\hline
  \raggedright{4 objects / game} &4.88 (2.20) &0.04 (0.01)  \\
  \hline 
    \end{tabular}
  \label{tab:captchaobjectuser}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf User Experience}
We conducted a post survey to evaluate how users felt after playing the games. The survey asked the participants to share their experiences while playing the games. We also asked the SUS questions and found the score to be 73.88, indicating high usability of such interfaces.  However, most participants did not notice any change in the speed or number of objects during the attack. 

We asked participants few likert (scale: 1 -  5) questions about their feedback on the usability of the games. Various aspects of this included - `` if the games were visually attractive'', `` Were the games pleasurable'' etc.  Forty seven percent participants felt the games to be visually attractive and 45\% said that it was pleasurable to play the games. This number depicts high possibility of making such interfaces more usable for relay attacks and also can be thought of as an indicator of humans being able to use such interfaces for relay attack. The Table~\ref{tab:usersus}, shows the average likert scores for various attributes of the game. We further enquired users, if they noticed change in speed or number of objects in the games and if this effected their game solving strategies. We found that 30\% found change in speed of objects whereas only 5\% noticed change in number of objects, as shown in Table \ref{tab:userother}.

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Usability attributes of the game}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Features} &  \bf Avg. Score\\
 \hline
 \hline
    \raggedright{Visually Attractive} & 3.18 (0.94)\\
 \hline
  \raggedright{Pleasurable } & 3.33 (0.96)\\
\hline
  \raggedright{Identity test } & 0.63 (1.11)\\
\hline
    \end{tabular}% For example,  
  \label{tab:usersus}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Speed and number of objects effect on users}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
  \textbf{Speed of objects} & (\%) \\
 \hline
    \raggedright{Moved faster} &30 \\
 \hline
  \raggedright{Moved slower } & 5 \\
\hline
  \raggedright{No change noticed } & 27.5\\
\hline

  \raggedright{Noticed both increase and decrease in speed} & 37.5\\
\hline
  \raggedright{Std. deviation} & 1.26 \\
\hline
 \textbf{Number of objects} & (\%) \\
 \hline
    \raggedright{Increased} & 47.5\\
 \hline
  \raggedright{Decreased } & 2.5\\
\hline
  \raggedright{No change noticed } & 22.5\\
\hline
  \raggedright{Noticed both increase and decrease in objects numbers} & 27.5\\
\hline
  \raggedright{Std. deviation} & 1.32 \\
\hline
    \end{tabular}% For example,  
  \label{tab:userother}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%


\smallskip \noindent {\bf Summary of Analysis:} Based on our analysis, we can
conclude that the DCG captcha categories tested in this work offer very good
usability, resulting in short completion times (less than 10 sec), very low
error rates (0\% per game completion, and less than 10\% per drag and drop
attempt), and high user ratings. We also find that increasing the object speed
and number of objects is likely to negatively affect the game performance, but
up to 6 objects and up to 40 FPS speed yield a high level of usability. 




==> usability-v2.tex <==
\section{Usability}
\label{sec:usability}

In this section, we report on a usability study of DCG captcha, including the
study design, goals, and testing process, as well as study results.

\subsection{Study Design, Goals, and Process}

Our study was undertaken by 40 participants. The corpus of participants
comprised primarily of undergraduate and graduate students from various
backgrounds. The demographics of the participants are shown in Table
\ref{tab:demographics-interviews} of the appendix. The study was
\textit{web-based} and comprised of three phases. The \textit{pre-study phase}
involved registering and briefly explaining the participants about the
protocols of the study.  In particular, the participants were shown ``consent
information,'' which they had to agree before proceeding with the study.  This
was followed by collecting participant demographics and then the participants
playing the different DCG captcha games.  This \textit{actual study phase}
attempted to mimic a realistic captcha scenario which typically involves
filling out a form followed by solving captcha. To avoid explicit priming,
however, we did not mention that the study is about captcha or security, but
rather indicated that it is about assessing the usability of a web interface.
The final, \textit{post-study phase} required the participants to respond to a
few questions about their experience and feedback on the games they played as
part of the interface. This comprised the standard SUS (Simple Usability Scale)
questions \cite{sus}, a widely used and highly reliable 10-item 5-point Likert
scale. It polls satisfaction with computer systems \cite{sus-chi}, in order to
assess usability of the method that was just tested.  Additionally, we asked
certain explicit questions related to the usability of the games (our
questionnaire set is provided in Appendix \ref{app:questions}). 

%The scenario given for study required users to evaluate a new interface for
%registering for a website followed by playing 20 games. 
During the actual study phase, each participant was asked to play 20
variations of the four DCG captcha categories implemented as discussed in Section
\ref{sec:design}. 
These variations were aimed at understanding how different parameters, i.e., object speed and
number of objects per game, affect the DCG captcha solving capability of the users. 
The order of the games presented to the participants was
counter-balanced for learning effects using the Latin Square design (a 20 x 20
Latin Square was used).
%These were presented to each participant using Latin square methodology. 
%We were not required to go through an IRB approval process before conducting
%the experiments. However, authors of this paper have previously been involved
%in studies with U.S. Institutional Review Board (IRB) approvals, and have
%applied similar practices in this study.  

The specific goal of our usability study was to evaluate and compare different DCG captcha games with
respect to the following factors:

\begin {enumerate}

\vspace{-2mm}
\item {\textit{Efficiency}: time taken to complete each game.}
\vspace{-2mm}
\item {\textit{Robustness}: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts.}
\vspace{-2mm}
\item \textit{Effect of Game Parameters}: the effect of the number of object and objects speeds on completion time and error rates
\vspace{-2mm}
\item {\textit{User Experience}: quantitative SUS ratings and qualitative feedback from the participants about their experience with the games.}
\vspace{-2mm}

\end {enumerate}

%Our study was conducted in a variety of campus venues including: student
%laboratories, cafes, student dorms/apartments, classrooms, ofÞce spaces and
%outdoor terraces .  After giving a brief overview of our study goals, we asked
%the participants to Þll out the background questionnaire to collect demographic
%information. This followed by a series 20 games to be played by the
%participants.Each user was asked to follow on-screen instructions in completing
%each task and was given a compensation of INR 75 for participating in the
%study.  
For each tested game, completion times, errors, actions and playcounts,
i.e., number of attempts made to successfully complete the games, were
established, and automatically logged by the our web-interface software.

\subsection{Study Results}

We now provide the results from our usability study. We
first consider various mechanical data, i.e., time to completion and error
rates. Then, we analyze perceived qualitative aspects of the methods based on
collected user ratings. 
%We nalize our interpretations by looking at all
%measures combined.


%\begin {itemize}

\smallskip \noindent {\bf Completion Time}: Table \ref{tab:captchaeff} shows
the time taken to complete the games per game category. Clearly, all games
turned out to be quite fast, lasting for less than 10 seconds on an average
(this far lower than our time out of 1 second).  We also found that users took
maximum time to solve the Animals game with an average time of 9.06 seconds,
whereas the other games took almost half of this time.  This might have been
due to increased semantic load on the users in the Animals game to identify
three target objects and then match them with the corresponding answer objects.
Moreover, we noticed a significant decrease in the solving time (3.83 sec) when
the target objects were decreased to 2 (i.e., in the Shapes game), and this
time was comparable to games which had 1 target object in the challenge (the
Ships game and the Parking game). Upon using a one-way repeated-measures ANOVA
test, we found significant difference among all 4 categories of games
($p<0.001$) on completion time.  On analyzing further using pairwise paired
t-tests, we found significant difference between the following pairs of games:
Animals and Parking ($p < 0.001$), Ships and Shapes ($p=0.0019$), Animals and Ships
($p<0.001$), Animals and Shapes ($p=0.00195$), and Parking and Shapes ($p=0.0005$).

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time per game type}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{2cm}|p{1.2cm}|}
   \hline
{\bf Game Type} &  \bf Completion Time (sec)& \bf Error Rate (\%)  \\
 &  \textit{mean (std dev)}& \textit{mean}    \\
 \hline
 \hline
    \raggedright{Place the Ships in the Sea } &4.74 (1.06) & 0.04 \\ %(0.02) \\
 \hline
  \raggedright{Feed the Animals} &9.06 (0.90)&0.05 \\ %(0.05)  \\
\hline
  \raggedright{Park the Boat} &4.37 (0.86) &0.09 \\%(0.03) %  \\
  \hline
  \raggedright{Match the Shapes} &5.23 (0.64)  &0.03 \\ %(0.02)\\
\hline 
    \end{tabular}
  \label{tab:captchaeff}
\end{center} 
}}
\vspace{-4mm}
\end{table}%


\smallskip \noindent {\bf Error Rates}:  An important result from our study is
that all the tested games yielded 100\% accuracy (overall error rate of 0\%).
In other words, none of the participant failed to complete any of the games
within the time out. This proves that DCG captchas can be highly robust in
practice.  

Next, we calculated the likelihood of exhibiting incorrect drag and drop
attempts. For example,  in the Animals game, an incorrect attempt would be to
feed the monkey with a flower instead of a banana.  We define the error rate in
this context as the number of incorrect objects (from the pool of probable
answer objects) dragged to the target area divided by the total of objects
dragged and dropped. The results are depicted in Table \ref{tab:captchaeff}.
Looking at the table, we observe that the Shape game yields the smallest average error
rate of 0.03\%.
% of incorrect attempts on an average for various speeds and number
%$of objects. 
This suggests that the visual matching task (as in the Shapes game)
is less error prone compared to the semantic matching task (as in the other
games). The game challenge which seemed most difficult
for the participants to solve was the Parking game (average error rate 0.09\%). Since
this was an empty target game, with the target region and the object region
having the same background, the participants may have found it a bit
difficult to perform the matching task.

%The goal of our usability study was to evaluate and compare different DCG captcha games with
%respect to the following factors:

%\begin {enumerate}
%\item {Efficiency: time taken to complete each game}
%\item {Robustness: likelihood of not completing the game as well as the likelihood of incorrect drag and drop attempts }
%\item {User Experience: quantitative SUS ratings and qualitative feedback from the participants.
%\end {enumerate}item 


\smallskip \noindent {\bf Effect of Object Speed}: Table
\ref{tab:captchaspeeduser} shows the performance of the game captchas in terms
of error rates and completion time as per different object speeds.  Looking at
the average error rates, we can see that 
%To evaluate the affect of speed on performance of the participants, we found
%the correlation between error rates and time taken to solve various game at
%different speed levels.  We also found that 
the maximum number of errors were committed at 10 FPS speed, which could be
because when objects move too slow, it may be a bit difficult to drag and drop
them. Looking at the average timings, we find that it took longest to complete
the games when the objects move at the fastest speed of 40 FPS, while 20 FPS
yielded fastest completion time followed by 10 FPS.  ANOVA test revealed
statistical difference among the completion time corresponding to three speeds
($p=0.006$). Further analyzing using the t-test, we found statistical
difference between the timing corresponding to following pair of speeds in
different game variants: 10 FPS and 20 FPS ($p<0.001$), and 20 FPS and 40 FPS
($p=0.0004$).  

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time per object speeds}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{2cm}|p{1.2cm}|}
   \hline
%{\bf Object Speed} &  \bf Avg. Play Time (sec) & \bf  Error Rate\\

{\bf Object Speed} &  \bf Completion Time (sec)& \bf Error Rate (\%)    \\
 &  \textit{mean (std dev)}& \textit{mean}    \\

 \hline
 \hline
    \raggedright{10 FPS } &5.80 (2.14) &0.06\\ %\\(0.06)  \\
 \hline
  \raggedright{20 FPS} &4.88 (2.20) &0.05 \\ %(0.04)  \\
\hline
  \raggedright{40 FPS} &6.50 (2.81) &0.04 \\ %(0.01)  \\
  \hline
    \end{tabular}
  \label{tab:captchaspeeduser}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Effect of Number of Objects}: Another aspect of the
usability analysis included testing the effect of increase in the number of
objects (noise / incorrect answer objects) on the overall game performance.
Table \ref{tab:captchaobjectuser} summarizes the error rates and completion
time against different number of objects. Here, we can see a clear pattern of
increase, albeit very minor, in average completion time and average rate with
increase in the number of objects. This is intuitive because increasing the
number of objects increases the cognitive load on the users which may slow down
the game play and introduce chances of errors.  ANOVA test did not indicate
this difference to be statistically significant, however.

\begin{table}[ht]
{\footnotesize{
  \begin{center} 
  \caption{Error rates and completion time per number of objects.}
        %\vspace{.2cm}
    \begin{tabular}{|p{3cm}|p{2cm}|p{1.2cm}|}
   \hline
%{\bf Number of Objects} &  \bf Error Rate (\%) & \bf Avg. Play Time (sec)\\
{\bf Number of Objects} &  \bf Completion Time (sec)& \bf Error Rate  (\%)   \\
 &  \textit{mean (std dev)}& \textit{mean}    \\

 \hline
 \hline
    \raggedright{ 6 objects / game } &6.52 (1.69) &0.06 \\ %(0.03) \\
 \hline
  \raggedright{5 objects / game} &5.34 (2.32) &0.05 \\ %(0.04) \\
\hline
  \raggedright{4 objects / game} &4.88 (2.20) &0.04 \\ %(0.01)  \\
  \hline 
    \end{tabular}
  \label{tab:captchaobjectuser}
\end{center} 
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf User Experience:}
%
Now, we analyze the data collected from the participants during the post-study
phase of the study. The average SUS score came out to be 73.88 (standard
deviation = xxx). Considering that industry average for SUS scores tends to
hover in the 60--70 range \cite{susmean}, the usability of game captchas can be
rated as high.
%Most participants did not notice any change in the
%speed or number of objects while playing the games. 

In addition to SUS, we asked the participants a few 5-point Likert scale
questions about the usability of the games. Specifically, we asked if the games
were ``visually attractive'' and ``pleasurable,'' and whether they would like
to use them in ``practice.'' The Table~\ref{tab:usersus}, shows the average
Likert scores for these attributes of the game. 
%`` if the games were visually attractive'', `` Were the games pleasurable''
%etc.  
We found that 47\% percent participants felt that the games were visually
attractive and 45\% said that it was pleasurable to play the games. These
numbers are largely positive and indicate the promising usability of the games.
%This number depicts high possibility of making such interfaces more usable for
%relay attacks and also can be thought of as an indicator of humans being able
%to use such interfaces for relay attack. 
We further enquired users if they noticed change in speed or number of objects
in the games. We found that 37.5\% found change (increase/decrease) in speed of
objects, whereas only 27.5\% noticed change in number of objects, as shown in
Table \ref{tab:userother}. This generally indicates that the change in the
number of objects and speed (within the limits we tested) was only mildly
noticeable and may not impact the overall usability of these games. This is
in line with our findings earlier based on the mechanical data. 

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{User feedback on game attributes}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
{\bf Attribute} &  \bf Likert Score\\
 &  \textit{mean (std dev)}\\
 \hline
 \hline
    \raggedright{Visually Attractive} & 3.18 (0.94)\\
 \hline
  \raggedright{Pleasurable } & 3.33 (0.96)\\
\hline
  \raggedright{Identity test } & 0.63 (1.11)\\
\hline
    \end{tabular}% For example,  
  \label{tab:usersus}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\begin{table}[ht]
{\footnotesize{
  \begin{center}
  \caption{Percentage of users noticing change in speed and number of objects}
        %\vspace{.2cm}
    \begin{tabular}{|p{4cm}|p{2cm}|}
   \hline
  \textbf{Object Speeds} & (\%) \\
 \hline
    \raggedright{Moved faster} &30 \\
 \hline
  \raggedright{Moved slower} & 5 \\
\hline
  \raggedright{No change noticed } & 27.5\\
\hline

  \raggedright{Noticed both increase and decrease in speed} & 37.5\\
%\hline
%  \raggedright{Std. deviation} & 1.26 \\
\hline
 \textbf{Number of objects} & (\%) \\
 \hline
    \raggedright{Increased} & 47.5\\
 \hline
  \raggedright{Decreased } & 2.5\\
\hline
  \raggedright{No change noticed } & 22.5\\
\hline
  \raggedright{Noticed both increase and decrease in objects numbers} & 27.5\\
%\hline
%  \raggedright{Std. deviation} & 1.32 \\
\hline
    \end{tabular}% For example,  
  \label{tab:userother}%
  \end{center}
}}
\vspace{-4mm}
\end{table}%

\smallskip \noindent {\bf Summary of Analysis:} Based on our analysis, we can
conclude that the DCG captcha categories tested in this work offer very good
usability, resulting in short completion times (less than 10 sec), very low
error rates (0\% per game completion, and less than 10\% per drag and drop
attempt), and high user ratings. We also find that increasing the object speed
and number of objects is likely to negatively affect the game performance, but
up to 6 objects and up to 40 FPS speed yield a high level of usability. 



